Adaptive manifold for imbalanced transductive few-shot learning

Transductive few-shot learning algorithms have showed substantially superior performance over their inductive counterparts by leveraging the unlabeled queries. However, the vast majority of such methods are evaluated on perfectly class-balanced benchmarks. It has been shown that they undergo remarkable drop in performance under a more realistic, imbalanced setting. To this end, we propose a novel algorithm to address imbalanced transductive few-shot learning, named Adaptive Manifold. Our method exploits the underlying manifold of the labeled support examples and unlabeled queries by using manifold similarity to predict the class probability distribution per query. It is parameterized by one centroid per class as well as a set of graph-specific parameters that determine the manifold. All parameters are optimized through a loss function that can be tuned towards class-balanced or imbalanced distributions. The manifold similarity shows substantial improvement over Euclidean distance, especially in the 1-shot setting. Our algorithm outperforms or is on par with other state of the art methods in three benchmark datasets, namely miniImageNet, tieredImageNet and CUB, and three different backbones, namely ResNet-18, WideResNet-28-10 and DenseNet-121. In certain cases, our algorithm outperforms the previous state of the art by as much as 4.2%.

==> tex/abstract-1.tex <==
%-------------------------------------------------------------------------------------------------------------------
\begin{abstract}
Transductive few-shot learning algorithms leveraging the unlabeled queries have showed substantially superior performance over their inductive counterparts. However, the vast majority of transductive few-shot learning algorithms test their performances on perfectly class-balanced benchmarks. It has been shown from \cite{alphaTIM} that these algorithms show remarkable drop in performance in a more realistic imbalanced transductive few-shot learning setting. To this we propose a novel algorithm tackling the imbalanced transductive few-shot learning, named differentiable manifold similarity centroids. Our algorithm exploits the underlying manifold structure of the labeled and unlabeled data by utilizing  manifold similarity to calculate the class probability of every query showing its superiority to euclidean distance. The manifold similarity centroids are updated using the loss function from \cite{alphaTIM} showing substantially superior performance than their euclidean counterpart especially in the 1-shot setting.

Our algorithm surpasses or is on par with other state of the art results in three benchmark datasets, namely \emph{mini}Imagenet, \emph{tiered}Imagenet and CUB and three different backbones, namely ResNet-18, WideResNet-28-10 and DenseNet. In certain cases our algorithm surpassing the other algorithms by as much as X$\%$ in 1-shot and Y$\%$ in 5-shot settings respectively. Our code can be accessed through this anonymous link: \url{XX}
\end{abstract}
%-------------------------------------------------------------------------------------------------------------------

==> tex/algo.tex <==
\footnotesize
\algrenewcommand\algorithmicindent{0.5em}%
    \begin{algorithmic}[1]
        \Require Access to $\{D_{base}, D_{novel}\}$ 
        \State Pre-train feature extractor, $f_\theta$, on $D_{base}$
        \State Sample a support set, $S$, and a querry set, $Q$, from $D_{novel}$
        \State extract feature embeddings, $v_i = f_{\theta}(x_i)$ for all samples, $x_i\in S \cup Q$
        \State pre-processing feature embeddings
		\For {iterate until all querries  from $Q$ are predicted}
	    	\State Graph construction, define affinity matrix, $A$, as \ref{eq:affinity}
	    	\State $W \gets A + A\tran$ %\comment{symmetric affinity}
            \State $\cW \gets D^{-1/2} W D^{-1/2}$ %\comment{symmetrically normalized affinity}
            \State Label Propagation: $Z \gets$ solve~\eq{lp} with CG
	    	\State Predict pseudolabels for querries using sinkhorn-knopp algorithm 
		    \State Label cleaning, choose the most likely example with the lowest loss
		    \State Augment support set, $S$, with selected pseudolabels
	    	\EndFor
    \end{algorithmic}


==> tex/experiments-1.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
\extdata{fig/data/sample}
\subsection{Setup}
\label{sec:setup}
\paragraph{Datasets}
We experiment on three commonly used few-shot learning benchmark datasets, namely \emph{mini}ImageNet~\cite{matchingNets}, \emph{tiered}ImageNet~\cite{sslmeta} and CUB~\cite{closerlook}.

\paragraph{Backbones}
We use three pre-trained backbones from the publicly available code provided by \cite{alphaTIM}, namely ResNet-18, WideResNet-28-10 (WRN-28-10) and \alert{DenseNet} as wellas the WRN-28-10 from \cite{ilpc}. All backbones were trained using the standard multi-class cross entropy loss on $D_{\base}$ over 90 epochs and using learning rate of 0.1 which is divided by 10 at epochs 45 and 66. Color jittering, random cropping and random horizontal flipping augmentations were used during training.

\paragraph{Tasks}
Unless otherwise stated, we consider N-way, K-shot tasks with N = 5 randomly sampled classes from $C_{\novel}$ and K = $\{1, 5\}$ random labeled examples for the support set $S$. The query set $Q$ contains a total of $M = 75$ query examples in total. In the balanced setting there are $\frac{M}{N}=\frac{75}{5} = 15$ queries per class. In the imbalanced setting the  total number of queries remains $M=75$ but the number of examples per class varies. We follow \cite{alphaTIM} to sample imbalanced tasks by modeling the proportion of examples from each class in $Q$ as a class proportion vector $\mathbf{\pi} = (\pi_1, \cdots, \pi_N)$ sampled from a Dirichlet distribution, $\mathrm{Dir}(\gamma)$ with parameter vector $\mathbf{\gamma}\vone_N$. We keep exactly the same setting as \cite{alphaTIM} and set $\gamma$=2.

\paragraph{Implementation details}
Our implementation is based in python using the Pytorch \cite{pytorch} framework. We carry out experiments for balanced and imbalanced transductive few-shot learning using the publicly available code provided by \cite{alphaTIM}\footnote{\url{https://github.com/oveilleux/Realistic_Transductive_Few_Shot}}. For further experiments regarding the balanced setting, we carry out experiments using the publicly available code provided from \cite{ilpc}\footnote{\url{https://github.com/MichalisLazarou/iLPC}}.

\paragraph{Hyperparameters}
For fair comparisons with respect to \cite{alphaTIM} we keep the common hyper-parameters the same, that is $\alpha$, $\eta$, $\tau$, $\lambda_1$, $\lambda_2$ and $\lambda_3$. We set $\eta=0.0001$,  $\tau = 15$ from \eq{softmax} and the $\alpha$ values from \eq{alpha-cond},\eq{alpha-entropy} equal to $2$ and $7$ in the 1-shot and 5-shot settings respectively. In the imbalanced setting we set $\lambda_1= \lambda_2=\lambda_3=1$ while in the balanced setting we set $\lambda_1=\lambda_3=1$ and $\lambda_2 = 10 $. Regarding the label propagation hyper-parameters, we initialize $k = 20$ and $\mathcal{B} = 0.8\vone_T^\textrm{T}\vone_T$ for the 1-shot setting and $k = 10$ and $\mathcal{B} = 0.9\vone_T^\textrm{T}\vone_T$ for the 5-shot setting respectively from equations \eq{edges} and \eq{lp} respectively. We set $\mathcal{G} = 1\vone_T^\textrm{T}\vone_T$ from equation \eq{lp}. \betalp, \sigmalp and $K$ were optimized on the validation set of \emph{mini}ImageNet. In order to avoid overfitting on hyperparameters, \emph{all hyper-parameters are kept constant across every dataset and backbone}.

\paragraph{Baselines}
 We compare our method with the state of the art methods regarding the imbalanced transductive few-shot learning. Since the state of the art in this setting is $\alpha$-TIM \cite{alphaTIM} we base our experiments on their publicly available code and compare against all available implemented methods. Regarding the balanced transductive few-shot learning we calculated the performances of all available algorithms provided in the publibly available code of \cite{alphaTIM}. Even though some methods with promising results in the balanced setting exist \cite{ilpc, ease} we did not carry out experiments on them since our is the imbalanced setting. The balanced experiments highlight the robustness of our algorithm and its superiority when compared against TIM \cite{TIM}.

\paragraph{Feature pre-processing}

\alert{(From method) We experiment with two commonly used pre-processing techniques to pre-process each vector in $V$, $\ell_2$-normalization and the pre-processing used in \cite{pt_map, ilpc} that we will refer to as \plc. $\ell_2$-normalization is simply defined as $\vv_i = \frac{\vv_i}{||\vv_i||_2}$ for every $\vv_i \in V$. \plc performs elementwise power transform to the $0.5$ for all $\vv_i \in V$  followed by $\ell_2$-normalization and centering using the mean of all vectors in $V$.}

As it was stated in section \ref{sec:problem} we explore the pre-processing techniques of $\ell_2$-normalization and \plc. We denote our method for the balanced setting using \plc pre-processing as \oursplc and using $\ell_2$-normalization as \ours. In the imbalanced setting we denote our method using \plc as $\alpha$-\oursplc and using $\ell_2$-normalization as $\alpha$-\ours.

TIM and $\alpha$-TIM use only $\ell_2$-normalization in their method. In order to provide fair and objective comparisons of our method against TIM~\cite{TIM} and $\alpha$-TIM~\cite{alphaTIM} we also calculated their performances when applying \plc pre-processing denoting them as TIM$_\textrm{plc}$ and $\alpha$-TIM$_{\textrm{plc}}$ respectively.

\paragraph{Guidance for experimental results}

In every table we denote the best performing results with bold regardless of the feature pre-processing used. However, since our work was influenced from \cite{TIM} and \cite{alphaTIM}, as a way to fair and objective comparisons we specifically compare our work with \cite{TIM} and \cite{alphaTIM} when the same feature pre-processing was used for both methods. In the tables that were calculated using the codebase from \cite{alphaTIM} we only report the mean accuracy since the accuracy was calculated over 10000 tasks following and that is the way \cite{alphaTIM} also reported their results. When using the codebase from \cite{ilpc}, we also report the 95$\%$ confidence interval since the results were calculated over 1000 tasks.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccccccccccccc}
\toprule
\mc{5}{\Th{Components}}          & \mc{4}{\Th{Imbalanced}}   & \mc{4}{\Th{Balanced}}              \\
     &      &      &         &             & \mc{2}{\Th{ResNet-18}}                   & \mc{2}{\Th{WRN-28-10}}      & \mc{2}{\Th{ResNet-18}}                   & \mc{2}{\Th{WRN-28-10}}              \\
\nnk & \mus & \sigmalp & \betalp & \plc &  1-shot              & 5-shot              & 1-shot              & 5-shot       & 1-shot              & 5-shot              & 1-shot              & 5-shot                    \\ \midrule
    &      &       &  &   & 60.21\ci{0.27}       &   74.31\ci{0.21}   &  63.34\ci{0.27}    & 76.22\ci{0.21}       & 59.09\ci{0.21}      & 71.54\ci{0.19}     & 62.38\ci{0.21}     & 73.46\ci{0.19} \\
\ch &      &      &  &   & 63.95\ci{0.27}     & 74.26\ci{0.21}      & 67.14\ci{0.27}      &  83.27\ci{0.16}    & 63.82\ci{0.22}      & 80.47\ci{0.15}     & 67.22\ci{0.21}      & 82.58\ci{0.15}  \\
\ch & \ch  &     &  &           & 68.51\ci{0.28}         &   81.23\ci{0.16}    &   71.16\ci{0.27}   & 84.69\ci{0.15}   & 73.43\ci{0.23}      & 84.40\ci{0.14}     & 75.94\ci{0.22}      & 86.51\ci{0.13}   \\
\ch &   \ch   & \ch     &  &        &   70.26\ci{0.29}    & 82.44\ci{0.17}     &   \tb{72.93}\ci{0.29}   & 84.72\ci{0.16}    & 75.59\ci{0.27}      & 84.85\ci{0.15}     & 78.71\ci{0.25}      &  86.99\ci{0.14} \\
\ch & \ch  &     &  \ch  &          & 66.30\ci{0.31}      & 82.43\ci{0.17}     &  67.87\ci{0.31}     & 84.63\ci{0.16}    & 74.89\ci{0.25}      & 84.57\ci{0.15}  & 77.72\ci{0.23}     & 86.70\ci{0.13}  \\
  \ch  & \ch  & \ch    & \ch & & 70.03\ci{0.30}      & 82.34\ci{0.17}     & 72.54\ci{0.29}     & 84.71\ci{0.16}  & 76.37\ci{0.28}      &  84.85\ci{0.15}       & 79.70\ci{0.82}      & 87.07\ci{0.14}    \\
    \ch  & \ch  & \ch    & \ch & \ch & \tb{70.03}\ci{0.30}      & \tb{83.27}\ci{0.17}     & 71.55\ci{0.29}     & \tb{85.71}\ci{16}    & \tb{77.46}\ci{0.27}      & \tb{85.47}\ci{0.14}     & \tb{81.05}\ci{0.26}     & \tb{87.85}\ci{0.13}  \\

\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Ablation study of algorithmic components} of both balanced and imbalanced versions of our method \ours on \emph{mini}ImageNet. \nnk: using $k$-nearest neighbour graph, otherwise a dense graph is used. \mus: adaptive class centroids. \sigmalp: adaptive \sigmalp. \betalp: adaptive \betalp. \plc: \plc pre-processing.}
\label{tab:ablation}
\end{table*}
%------------------------------------------------------------------------------


\subsection{Ablation study}
\subsubsection{Algorithmic components}
We ablate every component of our method both in the imbalanced and balanced settings. In the balanced setting we use the loss function in \eq{balanced} while in the imbalanced setting we use the loss function in \eq{imbalanced}. It is evident that using $k$-nearest neighbour graph gives significant performance over using a dense graph as it can be seen from the first and second rows of Table \ref{tab:ablation}. Also, adapting the centroids \mus by optimizing their embedding through \eq{imbalanced} or \eq{balanced} increases the performance substantially. Furthermore, adapting the centroids \mus along with manifold parameters \sigmalp and \betalp can enhance the performance even more especially in the balanced setting. Interestingly, adapting \mus with only \betalp seems to hinder the performance in the imbalanced setting when compared to adapting only \mus, nevertheless adapting \mus, \betalp and \sigmalp provide the best overall performance across both balanced and imbalanced settings. Additionally using \plc pre-processing provides further performance improvement in the balanced setting as well as the 5-shot imbalanced setting. Even though the 1-shot performance in the imbalanced setting is slightly degraded by using \plc the overall effect of \plc in every setting justifies its merits.

\subsubsection{Ablation on $\alpha$ hyper-parameter}
We can see from Figure \ref{fig:alpha_fig} the value of $\alpha$ has a lot more effect in the 1-shot setting than in the 5-shot setting. The optimal value of $\alpha$ is $\sim 2$ for the 1-shot while for 5-shot is $\sim 3$. We set $\alpha = 2$ for all of our 1-shot imbalanced experiments which is also the value that $\alpha$-TIM uses for their 1-shot experiments as well. In the 5-shot setting, since the effect of $\alpha>3$ is marginal we keep $\alpha = 7$ for all of our 5-shot experiments since it will also make the comparisons with $\alpha$-TIM more fair since they also use $\alpha = 7$ in their 5-shot experiments.
%-------------------------------------------------------------------------------------
\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=20,
    % x dir=reverse,
	xlabel={$\alpha$},
	ylabel={mean accuracy},
    legend style={at={(0.45,0.38)}},
	% legend pos={south east},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[violet, mark=*] table[x=alphavalues, y=oneshot] \alphagraph; \leg{1-shot \ours}
\addplot[brown, mark=*]  table[x=alphavalues,y=fiveshot]  \alphagraph; \leg{5-shot \ours}
\addplot[yellow, mark=*] table[x=alphavalues, y=timone] \alphagraph; \leg{1-shot $\alpha$-TIM}
\addplot[green, mark=*]  table[x=alphavalues,y=timfive]  \alphagraph; \leg{5-shot $\alpha$-TIM}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect of $\alpha$ for $\alpha$-\ours} on the 1-shot and 5-shot \emph{mini}ImageNet}
\label{fig:alpha_fig}
\end{figure}
%------------------------------------------------------------------------------


\subsection{Comparison of state of the art}

\subsubsection{Imbalanced transductive few-shot learning}
It can be seen from Tables \ref{tab:soa-imbalanced} and \ref{tab:imbalanced_cub} that our method achieves new state of the art performance using both backbones ResNet-18 and WRN-28-10 and under all three datasets of \emph{mini}ImageNet, \emph{tiered}ImageNet except on the 5-shot CUB with ResNet-18 whi. Impressively, the performance of our method substantially improves the state of the art in every 1-shot setting by as much as $4.3\%$ in the ResNet-18 CUB. While we can achieve state of the art performance even without the use of \plc pre-processing, \plc seems to provide a good performance trade-off between 1-shot and 5-shot performances since it improves the performance on the 5-shot but slightly degrades the 1-shot performance. In order to provide fair comparisons with $\alpha$-TIM we applied \plc pre-processing to $\alpha$-TIM however it can be seen from \ref{tab:soa-imbalanced} that its performance decreases.


%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
\Th{Method}                                        & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}     \\

                                               & 1-shot              & 5-shot & 1-shot              & 5-shot   \\ \midrule
                                       \mc{5}{\Th{ResNet-18}}  \\ \midrule

Entropy-min~\cite{entropy-min}              & 58.5     & 74.8    & 61.2     & 75.5\\
LR+ICI~\cite{lrici}                             & 58.7     & 73.5    &  74.6    &   85.1\\
PT-MAP~\cite{pt_map}                           & 60.1     & 67.1   & 64.1     & 70.0 \\
LaplacianShot~\cite{laplacianshot}             & 65.4     & 81.6   & 72.3     & 85.7 \\
BD-CSPN~\cite{BDCSPN}                 & 67.0     & 80.2   & 74.1     & 84.8 \\
TIM~\cite{TIM}                                & 67.3     & 79.8   & 74.1     & 84.1 \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}                   & 67.4     & 82.5    & 74.4    & 86.6\\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}    & 63.38    &   82.80   & 70.17     & 86.82\\ %\midrule
%------------------------------------------------------OFFICIAL DATA WITH THE 2 VARIATIONS---------------------------------------------------------
% \ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.30}     & 82.12\ci{0.17}   & 77.28\ci{0.30}     & 86.59\ci{0.18}         \\
% \ours($\beta=0.9, k=10$)               &    &   & 68.44\ci{0.29}     & 82.41\ci{0.17}   & 75.73\ci{0.29}     & 87.02\ci{0.18}         \\
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.29}     & 82.75\ci{0.17}   & 76.59\ci{0.29}      & 86.72\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 68.99\ci{0.29}     & 83.27\ci{0.17}   & 75.75\ci{0.28}    & 87.28\ci{0.17}         \\
%--------------------------------------------------------------------------------------------------------------------------------------------------
\rowcolor{LightCyan} $\alpha$-\ours                                     & \tb{70.03}     & 82.34   & \tb{77.28}     & 87.02 \\
\rowcolor{LightCyan} $\alpha$-\oursplc                    &  \tb{70.03}     & \tb{83.27}   & 76.59   & \tb{87.28} \\
\midrule
                                       \mc{5}{\Th{WRN-28-10}}  \\ \midrule
% Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & -     & - & -     & -       \\
% Baseline~\cite{closerlook}              &     &    & 62.2     & 81.9   & 63.5      & 83.8          \\
% Baseline++~\cite{closerlook}            &    &    & 64.5     & 82.1 & 68.0     & 84.2           \\
% Simpleshot~\cite{simpleshot}            &    &   & 66.2     & 82.4  & 69.6     & 84.7          \\
% \midrule
% MAML \cite{MAML}                         &  \multirow{11}*{WRN-28-10}  &  \multirow{11}*{Transdutive} & -     & -   & -     & -     \\
% Versa                                    &     &    & -     & -   & -     & -          \\
Entropy-min \cite{entropy-min}         & 60.4    & 76.2 & 62.9     & 77.3      \\
% LR+ICI~\cite{lrici}                      &    &    & -     & - & -     & -           \\
PT-MAP~\cite{pt_map}                         & 60.6     & 66.8   & 65.1     & 71.0  \\
LaplacianShot~\cite{laplacianshot}             & 68.1     & 83.2   & 73.5     & 86.8 \\
BD-CSPN~\cite{BDCSPN}                   & 70.4     & 82.3   &  75.4    & 85.9 \\
TIM~\cite{TIM}                                 & 69.8     & 81.6    & 75.8    & 85.4 \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}                   & 69.8     & 84.8     & 76.0   & 87.8 \\
%$\alpha$-TIM*~\cite{alphaTIM}                &   & 70.32\ci{0.28}     & 84.91\ci{0.16}    & 75.97\ci{0.28}     & 87.75\ci{0.18}  & -    & -   & -    & -     \\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}                  & 66.50     & 85.12    & 71.97     &  88.28\\ %\midrule
% \ours($\beta=0.8, k=20$)              &    &   & 72.54\ci{0.29}     & 84.17\ci{0.16}   & 78.90\ci{0.30}     & 87.63\ci{0.17}         \\
% \ours($\beta=0.9, k=10$)               &    &   & 71.21\ci{0.29}     & 84.71\ci{0.16}   & 77.25\ci{0.29}     & 88.05\ci{0.17}        \\
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 71.55\ci{0.29}     & 84.78\ci{0.16}   & 78.66\ci{0.29}     & 88.01\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 71.48\ci{0.28}     & 85.71\ci{0.16}   & 77.90\ci{0.27}     & 88.67\ci{0.17}         \\
\rowcolor{LightCyan} $\alpha$-\ours                              & \tb{72.54}     & 84.71  & \tb{78.90}     & 88.05\\

\rowcolor{LightCyan} $\alpha$-\oursplc                             & 71.55     & \tb{85.71}   & 78.66    & \tb{88.67} \\

\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}.}
\label{tab:soa-imbalanced}
\end{table}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
% \small
\centering
% \begin{adjustbox}{width=1\columnwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcc}
\toprule
\Th{Method} & \mc{2}{\Th{CUB}}       \\
           & 1-shot              & 5-shot         \\ \midrule
\mc{3}{\Th{ResNet-18}} \\ \midrule
% Baseline~\cite{closerlook}              &  \multirow{3}*{ResNet-18}  &  \multirow{3}*{Inductive}    & 64.6     & 86.9          \\
% Baseline++~\cite{closerlook}            &    &    & 69.4     & 87.5            \\
% Simpleshot~\cite{simpleshot}            &    &   & 70.6     & 87.5          \\
% \midrule
PT-MAP~\cite{pt_map}                    & 65.1     & 71.3      \\
Entropy-min~\cite{entropy-min}           & 67.5     & 82.9          \\
LaplacianShot~\cite{laplacianshot}       & 73.7     & 87.7           \\
BD-CSPN~\cite{BDCSPN}                   & 74.5     & 87.1           \\
TIM~\cite{TIM}                            & 74.8     & 86.9        \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}             & 75.7     & \tb{89.8}       \\
% *$\alpha$-TIM~\cite{alphaTIM}            &    &   & 76.57\ci{0.26}     & 90.03\ci{0.12}         \\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}        & 70.95   & 89.56   \\
% \midrule
\rowcolor{LightCyan} $\alpha$-\ours & \tb{80.00} & 89.62 \\
\rowcolor{LightCyan} $\alpha$-\oursplc & 79.02 & \tb{89.80} \\

% \ours($\beta=0.8, k=20$)                & 80.00\ci{0.28}     & 89.72\ci{0.12}           \\
% PLC+\ours($\beta=0.8, k=20$)            & 79.02\ci{0.28}     & 89.62\ci{0.12}          \\
% \ours($\beta=0.9, k=10$)                & 76.81\ci{0.28}     & 89.64\ci{0.12}           \\
% PLC+\ours($\beta=0.9, k=10$)           & 77.03\ci{0.27}     & 89.80\ci{0.12}           \\
\bottomrule

\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:imbalanced_cub}
\end{table}
%------------------------------------------------------------------------------

%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
 \Th{Method}                                      & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}        \\

                                               & 1-shot              & 5-shot & 1-shot              & 5-shot           \\ \midrule
                                       \mc{5}{\Th{ResNet-18}}  \\ \midrule

%Entropy-min~\cite{entropy-min}              & - & - & - & -        \\
PT-MAP~\cite{pt_map}                           & 76.88    & 85.18   & 82.89    & 88.64          \\
LaplacianShot~\cite{laplacianshot}             & 70.24    & 82.10   & 77.28    & 86.22          \\
BD-CSPN~\cite{BDCSPN}                           & 69.36    & 82.06   & 76.36    & 86.18         \\
TIM~\cite{TIM}                                & 73.81    & 84.91   & 80.13    & 88.61       \\
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 69.33    & 84.53  & 76.36   & 88.33 \\
%\midrule
%$\alpha$-TIM*~\cite{alphaTIM}                &   & 67.15\ci{0.28}     & 82.53\ci{0.17}    & 74.34\ci{0.28}     & 86.68\ci{0.18} & - & - & - & -        \\
\rowcolor{LightCyan} \ours                                             & 76.37 & 84.85 & 82.68 & 88.60    \\
\rowcolor{LightCyan} \oursplc                          & \tb{77.46} & \tb{85.47} & \tb{83.53} & \tb{89.06}       \\
\midrule
                                       \mc{5}{\Th{WRN-28-10}}  \\ \midrule
% Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & -     & - & -     & -       \\
% Baseline~\cite{closerlook}              &     &    & 62.2     & 81.9   & 63.5      & 83.8          \\
% Baseline++~\cite{closerlook}            &    &    & 64.5     & 82.1 & 68.0     & 84.2           \\
% Simpleshot~\cite{simpleshot}            &    &   & 66.2     & 82.4  & 69.6     & 84.7          \\
% \midrule
% MAML \cite{MAML}                         &  \multirow{11}*{WRN-28-10}  &  \multirow{11}*{Transdutive} & -     & -   & -     & -     \\
% Versa                                    &     &    & -     & -   & -     & -          \\
%Entropy-min \cite{entropy-min}         &  - & - & - & -           \\
PT-MAP~\cite{pt_map}                         &  80.35   & 87.37   & 84.84    & 89.86         \\
LaplacianShot~\cite{laplacianshot}             &  72.91    & 83.85   & 78.85    & 87.27         \\
BD-CSPN~\cite{BDCSPN}                   & 72.16   & 83.78   & 77.88   & 87.23       \\
TIM~\cite{TIM}                       &           77.78    & 87.43   & 82.28    & 89.84          \\
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 73.52    & 86.95   & 78.23    & 89.56 \\
%\midrule
\rowcolor{LightCyan} \ours                                             & 79.70 &  87.07 & 84.34 & 89.68   \\
\rowcolor{LightCyan} \oursplc                           & \tb{81.05} & \tb{87.85} & \tb{85.34} & \tb{90.28}       \\

%$\alpha$-TIM*~\cite{alphaTIM}                &   & 70.32\ci{0.28}     & 84.91\ci{0.16}    & 75.97\ci{0.28}     & 87.75\ci{0.18}  & -    & -   & -    & -     \\
% \ours($\beta=0.8, k=20$)              &    &   & 72.54\ci{0.29}     & 84.17\ci{0.16}   & 78.90\ci{0.30}     & 87.63\ci{0.17}         \\
% \ours($\beta=0.9, k=10$)               &    &   & 71.21\ci{0.29}     & 84.71\ci{0.16}   & 77.25\ci{0.29}     & 88.05\ci{0.17}        \\
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 71.55\ci{0.29}     & 84.78\ci{0.16}   & 78.66\ci{0.29}     & 88.01\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 71.48\ci{0.28}     & 85.71\ci{0.16}   & 77.90\ci{0.27}     & 88.67\ci{0.17}         \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. All results are calculated using the the publicly available code provided from \cite{alphaTIM}. }
\label{tab:soa-balanced}
\end{table}
%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------


%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcc}
\toprule
\Th{Method}                            & \mc{2}{\Th{CUB}}        \\
     & 1-shot              & 5-shot            \\ \midrule
% Protonet~\cite{prototypical}            & 64.51\ci{0.21}    & 86.91\ci{0.12}        \\
% Baseline~\cite{closerlook}               & 64.51\ci{0.21}    & 87.02\ci{0.11}         \\
% Baseline++~\cite{closerlook}            & 69.47\ci{0.21}    & 87.63\ci{0.11}         \\
% Simpleshot~\cite{simpleshot}            & 70.53\ci{0.20}    & 87.60\ci{0.11}        \\
% \midrule
%Entropy-min~\cite{entropy-min}          & -    & -         \\
PT-MAP~\cite{pt_map}                    & 86.05    & 91.28        \\
LaplacianShot~\cite{laplacianshot}      & 79.55    & 88.96         \\
BD-CSPN~\cite{BDCSPN}                   & 78.52   & 89.02        \\
TIM~\cite{TIM}                          & 82.87     & 91.58       \\
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 77.69    & 91.17 \\
%\midrule
\rowcolor{LightCyan} \ours                                   & 85.88         & 91.35\\
\rowcolor{LightCyan} \oursplc                                & \tb{86.80}         & \tb{91.68} \\
% \midrule
% \ours($\beta=0.8, k=20$)                & 85.88\ci{0.24}    & 91.16\ci{0.10}        \\
% \ours($\beta=0.9, k=10$)                & 84.30\ci{0.23}    & 91.35\ci{0.10}        \\
% PLC+\ours($\beta=0.8, k=20$)            & 86.80\ci{0.23}    & 91.68\ci{0.10}        \\
% PLC+\ours($\beta=0.9, k=10$)            & 85.19\ci{0.23}    & 91.86\ci{0.10}         \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-balanced_cub}
\end{table}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

\subsubsection{Balanced transductive few-shot learning}
It can be seen from tables \ref{tab:soa-balanced} and \ref{tab:soa-balanced_cub} that \oursplc can outperform every other baseline with its closest competitor being PT-MAP~\cite{pt_map}. It should be noted that PT-MAP also uses \plc pre-processing meaning that our superiority is not based on the pre-processing. Comparing \ours against TIM it can be seen that we can significantly outperform them in all settings when \plc is used. Interestingly, TIM's performance is degraded through the use of \plc while \ours is improved which shows the robustness of our method. Even without \plc, \ours significantly outperforms TIM in the 1-shot setting by $\sim 2-4\%$ while performing on par or slightly worse by $\sim 0.1-0.3\%$ on the 5-shot setting.

Since the codebase provided by \cite{alphaTIM} does not provide some of the state of the art methods in the balanced transductive few-shot learning such as \cite{ilpc} and \cite{ease}, we use the codebase provided by \cite{ilpc} using their publicly available code to compare our performance against the best state of the art methods in the balanced setting using. We use the available pre-trained WRN-28-10 network provided by \cite{ilpc} and compare \ours, TIM, EASE \cite{ease}, PT+MAP \cite{pt_map} and iLPC \cite{ilpc}. Since the results of PT+MAP and iLPC were provided through this code base we did not re-calculate their performance, we simply calculated the performances of \ours, TIM and EASE with and without the use of \plc. It should be noted that PT+MAP and iLPC use \plc pre-processing as part of their method. It can be seen from table \ref{tab:trans_balanced_ilpc}

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \color{red}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccccc}
\toprule
\Th{Method}                             & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\
                                               & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
                                        \mc{9}{\Th{WRN-28-10}} \\
\midrule
% LaplacianShot~\cite{laplacianshot}  & 74.86\ci{0.19} & 84.13\ci{0.14} & 80.18\ci{0.21} & 87.56\ci{0.15} & - &- & -& -\\
%\rowcolor{LightGray}EASE+SIAMESE~\cite{ease}*          & 83.00\ci{0.21} & 88.92\ci{0.13} & \tb{88.96}\ci{0.23} & \tb{92.63}\ci{0.13} & \tb{87.60}\ci{0.23} & 90.60\ci{0.16} & \tb{91.68}\ci{0.19} & 94.12\ci{0.09}\\ \midrule
PT+MAP~\cite{pt_map}                    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
\ilpc~\cite{ilpc}          & 83.05\ci{0.79} & 88.82\ci{0.42} & 88.50\ci{0.75} & 92.46\ci{0.42} & 86.51\ci{0.75} & 90.60\ci{0.48} & 91.03\ci{0.63} & 94.11\ci{0.30}\\
EASE+SIAMESE~\cite{ease}          & 83.44\ci{0.77} & 88.66\ci{0.43} & \tb{88.69}\ci{0.73} & 92.47\ci{0.41} & 86.71\ci{0.77} & 90.28\ci{0.51} & 91.44\ci{0.63} & 93.85\ci{0.32} \\
EASE+SIAMESE$_\textrm{plc}$~\cite{ease}          & 82.13\ci{0.81} & 87.34\ci{0.46}& 88.42\ci{0.73} & 92.19\ci{0.41} & 86.74\ci{0.78} & 90.22\ci{0.51} & \tb{91.49}\ci{0.63} & 93.32\ci{0.32} \\
% %TIM \cite{TIM}      &     & 77.8\cip & 87.4\cip  & 82.1\cip & 89.8\cip & - & - & - & -\\
TIM \cite{TIM}        & 77.65\ci{0.72} & 88.21\ci{0.40}  & 83.88\ci{0.74} & 91.89\ci{0.41} & 82.63\ci{0.70} & 90.28\ci{0.46} & 87.50\ci{0.62} & 93.59\ci{0.30}\\
TIM$_{\textrm{plc}}$ \cite{TIM}    & 75.77\ci{0.67} & 88.37\ci{0.40}  & 83.22\ci{0.70} & 92.13\ci{0.40} & 80.52\ci{0.70} & 90.25\ci{0.46} & 85.58\ci{0.61} & 93.48\ci{0.31}\\
\rowcolor{LightCyan} \ours            & 80.97\ci{0.82} & 87.75\ci{0.42}  & 86.51\ci{0.78} & 91.81\ci{0.43} & 86.25\ci{0.74} & 90.14\ci{0.47} & 90.53\ci{0.65} & 93.47\ci{0.30}\\
\rowcolor{LightCyan} \oursplc        & \tb{83.53}\ci{0.73} & \tb{89.06}\ci{0.40}  & 88.28\ci{0.73} &  \tb{92.61}\ci{0.39} & \tb{87.04}\ci{0.74} & \tb{90.78}\ci{0.46} & 91.46\ci{0.60} & \tb{94.13}\ci{0.29} \\\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Balanced transductive inference state of the art}. *: results are reported from \cite{ease}. All the rest of the results were calculated using the codebase provided by \cite{ilpc}}
\label{tab:trans_balanced_ilpc}
\end{table*}
%---------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------}

\subsection{Effect of unlabeled data}
%We argue that the slight performance deficit in the balanced 5-shot setting without \plc is simply a benchmarking limitation.
We investigate the effect of unlabeled data comparing $\alpha$-\ours against $\alpha$-TIM. It can be seen from figure \ref{fig:num-unlabeled} regarding the 1-shot setting that when using more unlabeled data, $M>275$, $\alpha$-\ours not only outperforms $\alpha$-TIM but the performance gap also increases going from $\sim 2.5\%$ when $M=75$ to $\sim 4.5\%$ when $M=500$.  This can be attributed to the fact that $\alpha$-\ours leverages the manifold structure through the $k$-nearest neighbour graph while $\alpha$-TIM works in euclidean space.


\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=67,
    % x dir=reverse,
	xlabel={number of unlabeled queries},
	ylabel={mean accuracy},
    % legend style={at={(0.45,0.38)}},
	legend pos={north west},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[blue, mark=*] table[x=unlabeled, y=ours] \unlabeledone; \leg{$\alpha$-\ours}
\addplot[red, mark=*]  table[x=unlabeled,y=tim]  \unlabeledone; \leg{$\alpha$-TIM}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect of number of unlaled data on $\alpha$-\ours and $\alpha$-TIM} on the 1-shot \emph{mini}ImageNet}
\label{fig:num-unlabeled}
\end{figure}
%------------------------------------------------------------------------------


\subsection{Robustness against imbalance}

We investigate the effect of increasing the class imbalance in $Q$ by decreasing the value of the $\gamma \vone_N$ used in $\mathrm{Dir}(\gamma)$. As it can be seen in figure \ref{fig:gamma_fig} when comparing $\alpha$-\ours and $\alpha$-TIM in the 1-shot \emph{mini}ImageNet it can be seen that $\alpha$-\ours consistently outperforms $\alpha$-TIM even when the class imbalanced is increased.

\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=56,
    x dir=reverse,
	xlabel={$\gamma$},
	ylabel={mean accuracy},
    % legend style={at={(0.45,0.38)}},
	legend pos={south west},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[blue, mark=*] table[x=dirichlet, y=ours] \alphadirichlet; \leg{$\alpha$-\ours}
\addplot[red, mark=*]  table[x=dirichlet,y=tim]  \alphadirichlet; \leg{$\alpha$-TIM}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect of $\gamma$ for $\textrm{Dir}(\gamma)$} on the 1-shot \emph{mini}ImageNet}
\label{fig:gamma_fig}
\end{figure}
%------------------------------------------------------------------------------

\subsection{Other backbones}
It can be seen from Table \ref{tab:densenet} that the best version of our method, \oursplc outperforms $\alpha$-TIM and $\alpha$-TIM$_\mathrm{plc}$ in both 1-shot and 5-shot settings. As with the previous experiments, a significant gap in performance of $\sim 3.5\%$ can be seen in the 1-shot setting.
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lcccc}
\toprule
\Th{Method}   & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}} \\
           & 1-shot              & 5-shot              & 1-shot              & 5-shot\\ \midrule
                        \mc{5}{\Th{Imbalanced - DenseNet-121}} \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}     & 70.41  & 85.58 &  - & -     \\
$\alpha$-TIM$_{\textrm{plc}}$~\cite{alphaTIM}     & 67.56  & 86.26 &  - & -     \\
$\alpha$-\ours              & 73.53      & 85.19 &  - & -  \\
$\alpha$-\oursplc           & \tb{73.95}     & \tb{86.80} &  - & -  \\ %\midrule
%                         \mc{5}{\Th{Balanced - DenseNet-121}} \\ \midrule
% TIM~\cite{TIM}     & -      & - &  - & -     \\
% \ours              & -      & - &  - & -  \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference}, using the standard settings and Densenet-121 backbone}
\label{tab:densenet}
\end{table}
%-----------------------------------------------------------------------------















% %------------------------------------------------------------------------------
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{5pt}
% \begin{tabular}{lccccc}
% \toprule
% \Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}       \\
%                                         &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                     \\ \midrule
% LR+ICI~\cite{lrici}*                    & ResNet-12A   & -     & -      & -      & -          \\
% CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12   & -     & -      & -      & -               \\
% DPGN~\cite{DPGN}                        & ResNet-12    & -     & -      & -      & -        \\
% MCT (instance)~\cite{mct}               & ResNet-12B   & -     & -      & -      & -          \\
% \midrule
% EP~\cite{embeddingpropagation}          & WRN-28-10    & -     & -      & -      & -                  \\
% SIB~\cite{SIB}$\dagger$                 & WRN-28-10    & -     & -      & -      & -                    \\
% SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & -     & -      & -      & -                     \\
% LaplacianShot~\cite{laplacianshot} & WRN-28-10 & -     & -      & -      & -  \\
% PT+MAP~\cite{pt_map}*                   & WRN-28-10   & -     & -      & -      & -    \\
%  \\ \bottomrule
% \end{tabular}
% \vspace{6pt}
% \caption{\emph{Transductive inference state of the art}. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
% \label{tab:soa-trans}
% \end{table}
% %------------------------------------------------------------------------------


% %------------------------------------------------------------------------------
% % \extdata{fig/data/sample}
% \begin{figure}
% % \extfig{pca}
% % {
% \begin{tikzpicture}
% \begin{axis}[
% 	width=\linewidth,
% 	height=0.5\linewidth,
% 	font=\small,
% 	ymin=67.2,
%     x dir=reverse,
% 	xlabel={shots},
% 	ylabel={mean accuracy},
% 	legend pos={south west},
% ]
% % \addplot [black, domain=0:3.5] {25*x^0.2};
% \addplot[blue, mark=*] table[x=shots,y=ours] \lowshot; \leg{$\alpha$-\ours (ours)}
% % \addplot[red, mark=*]  table[x=shots,y=tim]  \lowshot; \leg{$\alpha$-TIM}
% \end{axis}
% \end{tikzpicture}
% % }
% \caption{michalis}
% \label{fig:low_shot}
% \end{figure}
%------------------------------------------------------------------------------


==> tex/experiments_not_compiling.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
\extdata{fig/data/sample}

\subsection{Setup}
\label{sec:setup}
\paragraph{Datasets}
We experiment on three commonly used few-shot learning benchmark datasets, namely \emph{mini}ImageNet~\cite{matchingNets}, \emph{tiered}ImageNet~\cite{sslmeta} and CUB~\cite{closerlook}.

\paragraph{Backbones}
We use three pre-trained backbones from the publicly available code provided by \cite{alphaTIM}\footnote{\url{https://github.com/oveilleux/Realistic_Transductive_Few_Shot}}, namely ResNet-18, WideResNet-28-10 (WRN-28-10) and \alert{DenseNet}. All backbones were trained using the standard multi-class cross entropy loss on $D_{\base}$ over 90 epochs and using learning rate of 0.1 which is divided by 10 at epochs 45 and 66. Color jittering, random cropping and random horizontal flipping augmentations were used during training.

\paragraph{Tasks}
Unless otherwise stated, we consider N-way, K-shot tasks with N = 5 randomly sampled classes from $C_{\novel}$ and K = $\{1, 5\}$ random labeled examples for the support set $S$. The query set $Q$ contains a total of $M = 75$ query examples in total. In the balanced setting there are $\frac{M}{N}=\frac{75}{5} = 15$ queries per class. In the imbalanced setting the  total number of queries remains $M=75$ but the number of examples per class varies. We follow \cite{alphaTIM} to sample imbalanced tasks by modeling the proportion of examples from each class in $Q$ as a class proportion vector $\mathbf{\pi} = (\pi_1, \cdots, \pi_N)$ sampled from a Dirichlet distribution, $\mathrm{Dir}(\gamma)$ with parameter vector $\mathbf{\gamma}\vone_N$. We keep exactly the same setting as \cite{alphaTIM} and set $\gamma$=2.

\paragraph{Implementation details}
Our implementation is based in python using the Pytorch \cite{pytorch} framework. We carry out our experiments using the code from \cite{alphaTIM}.

\paragraph{Hyperparameters}
For fair comparisons with respect to \cite{alphaTIM} we keep exactly the same hyper-parameters in the adaptation procedure, that is we keep the learning rate $\eta=0.0001$ and the $\alpha$ values from \eq{alpha_MI} equal to $2$ and $7$ in the 1-shot and 5-shot settings respectively. We set $\tau = 15$ from \eq{softmax}.  We initialize all values of $\mathcal{B} = 0.8$ and $K = 20$ for the 1-shot setting and $\mathcal{B} = 0.9$ and $K = 10$ for the 5-shot setting respectively and set all values of $\mathcal{G}$ equal to 1. \betalp, \sigmalp and $K$ were optimized on the validation set of \emph{mini}ImageNet. In order to avoid overfitting on hyperparameters, \emph{\textbf{all hyper-parameters are kept constant across every dataset and backbone}}.

\paragraph{Baselines}
 We compare our method with the state of the art methods regarding the imbalanced transductive few-shot learning. Since the state of the art in this setting is $\alpha$-TIM \cite{alphaTIM} we base our experiments on their publicly available code and compare against all available implemented methods. Regarding the balanced transductive few-shot learning we calculated the performances of all available algorithms provided in the publibly available code of \cite{alphaTIM}. Even though some methods with promising results in the balanced setting exist \cite{ilpc, ease} we did not carry out experiments on them since our is the imbalanced setting. The balanced experiments highlight the robustness of our algorithm and its superiority when compared against TIM \cite{TIM}.

\paragraph{Feature pre-processing}
As it was stated in section \ref{sec:embeddings} we explore the pre-processing techniques of $\ell_2$-normalization and \plc. We denote our method for the balanced setting using \plc pre-processing as \oursplc and using $\ell_2$-normalization as \ours. In the imbalanced setting we denote our method using \plc as $\alpha$-\oursplc and using $\ell_2$-normalization as $\alpha$-\ours. 

TIM and $\alpha$-TIM use only $\ell_2$-normalization in their method. In order to provide fair and objective comparisons of our method against TIM~\cite{TIM} and $\alpha$-TIM~\cite{alphaTIM} we also calculated their performances when applying \plc pre-processing denoting them as TIM$_\textrm{plc}$ and $\alpha$-TIM$_{\textrm{plc}}$ respectively.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccccccccccccc}
\toprule
\mc{5}{\Th{Components}}          & \mc{4}{\Th{Imbalanced}}   & \mc{4}{\Th{Balanced}}              \\ 
     &      &      &         &             & \mc{2}{\Th{ResNet-18}}                   & \mc{2}{\Th{WRN-28-10}}      & \mc{2}{\Th{ResNet-18}}                   & \mc{2}{\Th{WRN-28-10}}              \\ 
\nnk & \mus & \sigmalp & \betalp & \plc &  1-shot              & 5-shot              & 1-shot              & 5-shot       & 1-shot              & 5-shot              & 1-shot              & 5-shot                    \\ \midrule
    &      &       &  &   & 60.21\ci{0.27}       &   74.31\ci{0.21}   &  63.34\ci{0.27}    & 76.22\ci{0.21}       & 59.09\ci{0.21}      & 71.54\ci{0.19}     & 62.38\ci{0.21}     & 73.46\ci{0.19} \\ 
\ch &      &      &  &   & 63.95\ci{0.27}     & 74.26\ci{0.21}      & 67.14\ci{0.27}      &  83.27\ci{0.16}    & 63.82\ci{0.22}      & 80.47\ci{0.15}     & 67.22\ci{0.21}      & 82.58\ci{0.15}  \\ 
\ch & \ch  &     &  &           & 68.51\ci{0.28}         &   81.23\ci{0.16}    &   71.16\ci{0.27}   & 84.69\ci{0.15}   & 73.43\ci{0.23}      & 84.40\ci{0.14}     & 75.94\ci{0.22}      & 86.51\ci{0.13}   \\
\ch &   \ch   & \ch     &  &        &   70.26\ci{0.29}    & 82.44\ci{0.17}     &   \tb{72.93}\ci{0.29}   & 84.72\ci{0.16}    & 75.59\ci{0.27}      & 84.85\ci{0.15}     & 78.71\ci{0.25}      &  86.99\ci{0.14} \\ 
\ch & \ch  &     &  \ch  &          & 66.30\ci{0.31}      & 82.43\ci{0.17}     &  67.87\ci{0.31}     & 84.63\ci{0.16}    & 74.89\ci{0.25}      & 84.57\ci{0.15}  & 77.72\ci{0.23}     & 86.70\ci{0.13}  \\
  \ch  & \ch  & \ch    & \ch & & 70.03\ci{0.30}      & 82.75\ci{0.17}     & 72.54\ci{0.29}     & 84.71\ci{0.16}  & 76.37\ci{0.28}      &  84.85\ci{0.15}       & 79.70\ci{0.82}      & 87.07\ci{0.14}    \\
    \ch  & \ch  & \ch    & \ch & \ch & \tb{70.03}\ci{0.30}      & \tb{83.27}\ci{0.17}     & 71.55\ci{0.29}     & \tb{85.71}\ci{16}    & \tb{77.46}\ci{0.27}      & \tb{85.47}\ci{0.14}     & \tb{81.05}\ci{0.26}     & \tb{87.85}\ci{0.13}  \\

\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Ablation study of algorithmic components} of both balanced and imbalanced versions of our method \ours on \emph{mini}ImageNet. \nnk: using $k$-nearest neighbour graph, otherwise a dense graph is used. \mus: adaptive class centroids. \sigmalp: adaptive \sigmalp. \betalp: adaptive \betalp. \plc: \plc pre-processing.}
\label{tab:ablation}
\end{table*}
%------------------------------------------------------------------------------


\subsection{Ablation study}
We ablate every component of our method both in the imbalanced and balanced settings. In the balanced setting we use the loss function in \eq{balanced} while in the imbalanced setting we use the loss function in \eq{imbalanced}. It is evident that using $k$-nearest neighbour graph gives significant performance over using a dense graph as it can be seen from the first and second rows of Table \ref{tab:ablation}. Also, adapting the centroids \mus by optimizing their embedding through \eq{imbalanced} or \eq{balanced} increases the performance substantially. Furthermore, adapting the centroids \mus along with manifold parameters \sigmalp and \betalp can enhance the performance even more. Interestingly, adapting \mus and \betalp only seems to hinder the performance in the imbalanced setting when compared to adapting only \mus, nevertheless adapting \mus, \betalp and \sigmalp provide the best overall performance across both balanced and imbalanced settings. Additionally using \plc pre-processing provides further performance improvement in the balanced setting as well as the 5-shot imbalanced setting. Even though the 1-shot performance in the imbalanced setting is slightly degraded by using \plc the overall effect of \plc in every setting justifies its merits.


\subsection{Comparison of state of the art}

\subsubsection{Imbalanced transductive few-shot learning}
It can be seen from Tables \ref{tab:soa-imbalanced} and \ref{tab:imbalanced_cub} that our method achieves new state of the art performance using both backbones ResNet-18 and WRN-28-10 and under all three datasets of \emph{mini}ImageNet, \emph{tiered}ImageNet except on the 5-shot CUB with ResNet-18 whi. Impressively, the performance of our method substantially improves the state of the art in every 1-shot setting by as much as $4.3\%$ in the ResNet-18 CUB. While we can achieve state of the art performance even without the use of \plc pre-processing, \plc seems to provide a good performance trade-off between 1-shot and 5-shot performances since it improves the performance on the 5-shot but slightly degrades the 1-shot performance. In order to provide fair comparisons with $\alpha$-TIM we applied \plc pre-processing to $\alpha$-TIM however it can be seen from \ref{tab:soa-imbalanced} that its performance decreases.


%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
\Th{Method}                                        & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}     \\ 

                                               & 1-shot              & 5-shot & 1-shot              & 5-shot   \\ \midrule
                                       \mc{5}{\Th{ResNet-18}}  \\ \midrule
                                       
Entropy-min~\cite{entropy-min}              & 58.5     & 74.8    & 61.2     & 75.5\\
LR+ICI~\cite{lrici}                             & 58.7     & 73.5    &  74.6    &   85.1\\
PT-MAP~\cite{pt_map}                           & 60.1     & 67.1   & 64.1     & 70.0 \\
LaplacianShot~\cite{laplacianshot}             & 65.4     & 81.6   & 72.3     & 85.7 \\
BD-CSPN~\cite{BDCSPN}                 & 67.0     & 80.2   & 74.1     & 84.8 \\
TIM~\cite{TIM}                                & 67.3     & 79.8   & 74.1     & 84.1 \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}                   & 67.4     & 82.5    & 74.4    & 86.6\\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}    & 63.38    &   82.80   & 70.17     & 86.82\\ %\midrule
%------------------------------------------------------OFFICIAL DATA WITH THE 2 VARIATIONS---------------------------------------------------------
% \ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.30}     & 82.12\ci{0.17}   & 77.28\ci{0.30}     & 86.59\ci{0.18}         \\  
% \ours($\beta=0.9, k=10$)               &    &   & 68.44\ci{0.29}     & 82.41\ci{0.17}   & 75.73\ci{0.29}     & 87.02\ci{0.18}         \\ 
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.29}     & 82.75\ci{0.17}   & 76.59\ci{0.29}      & 86.72\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 68.99\ci{0.29}     & 83.27\ci{0.17}   & 75.75\ci{0.28}    & 87.28\ci{0.17}         \\
%--------------------------------------------------------------------------------------------------------------------------------------------------
\rowcolor{LightCyan} $\alpha$-\ours                                     & \tb{70.03}     & 82.75   & \tb{77.28}     & 87.02 \\  
\rowcolor{LightCyan} $\alpha$-\oursplc                    &  \tb{70.03}     & \tb{83.27}   & 76.59   & \tb{87.28} \\ 
\midrule
                                       \mc{5}{\Th{WRN-28-10}}  \\ \midrule
% Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & -     & - & -     & -       \\
% Baseline~\cite{closerlook}              &     &    & 62.2     & 81.9   & 63.5      & 83.8          \\
% Baseline++~\cite{closerlook}            &    &    & 64.5     & 82.1 & 68.0     & 84.2           \\
% Simpleshot~\cite{simpleshot}            &    &   & 66.2     & 82.4  & 69.6     & 84.7          \\
% \midrule
% MAML \cite{MAML}                         &  \multirow{11}*{WRN-28-10}  &  \multirow{11}*{Transdutive} & -     & -   & -     & -     \\
% Versa                                    &     &    & -     & -   & -     & -          \\
Entropy-min \cite{entropy-min}         & 60.4    & 76.2 & 62.9     & 77.3      \\
% LR+ICI~\cite{lrici}                      &    &    & -     & - & -     & -           \\
PT-MAP~\cite{pt_map}                         & 60.6     & 66.8   & 65.1     & 71.0  \\
LaplacianShot~\cite{laplacianshot}             & 68.1     & 83.2   & 73.5     & 86.8 \\
BD-CSPN~\cite{BDCSPN}                   & 70.4     & 82.3   &  75.4    & 85.9 \\ 
TIM~\cite{TIM}                                 & 69.8     & 81.6    & 75.8    & 85.4 \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}                   & 69.8     & 84.8     & 76.0   & 87.8 \\
%$\alpha$-TIM*~\cite{alphaTIM}                &   & 70.32\ci{0.28}     & 84.91\ci{0.16}    & 75.97\ci{0.28}     & 87.75\ci{0.18}  & -    & -   & -    & -     \\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}                  & 66.50     & 85.12    & 71.97     &  88.28\\ %\midrule
% \ours($\beta=0.8, k=20$)              &    &   & 72.54\ci{0.29}     & 84.17\ci{0.16}   & 78.90\ci{0.30}     & 87.63\ci{0.17}         \\  
% \ours($\beta=0.9, k=10$)               &    &   & 71.21\ci{0.29}     & 84.71\ci{0.16}   & 77.25\ci{0.29}     & 88.05\ci{0.17}        \\ 
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 71.55\ci{0.29}     & 84.78\ci{0.16}   & 78.66\ci{0.29}     & 88.01\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 71.48\ci{0.28}     & 85.71\ci{0.16}   & 77.90\ci{0.27}     & 88.67\ci{0.17}         \\  
\rowcolor{LightCyan} $\alpha$-\ours                              & \tb{72.54}     & 84.71  & \tb{78.90}     & 88.05\\  

\rowcolor{LightCyan} $\alpha$-\oursplc                             & 71.55     & \tb{85.71}   & 78.66    & \tb{88.67} \\

\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}.}
\label{tab:soa-imbalanced}
\end{table}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
% \small
\centering
% \begin{adjustbox}{width=1\columnwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcc}
\toprule
\Th{Method} & \mc{2}{\Th{CUB}}       \\ 
           & 1-shot              & 5-shot         \\ \midrule
\mc{3}{\Th{ResNet-18}} \\ \midrule
% Baseline~\cite{closerlook}              &  \multirow{3}*{ResNet-18}  &  \multirow{3}*{Inductive}    & 64.6     & 86.9          \\
% Baseline++~\cite{closerlook}            &    &    & 69.4     & 87.5            \\
% Simpleshot~\cite{simpleshot}            &    &   & 70.6     & 87.5          \\
% \midrule
PT-MAP~\cite{pt_map}                    & 65.1     & 71.3      \\
Entropy-min~\cite{entropy-min}           & 67.5     & 82.9          \\
LaplacianShot~\cite{laplacianshot}       & 73.7     & 87.7           \\
BD-CSPN~\cite{BDCSPN}                   & 74.5     & 87.1           \\
TIM~\cite{TIM}                            & 74.8     & 86.9        \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}             & 75.7     & \tb{89.8}       \\
% *$\alpha$-TIM~\cite{alphaTIM}            &    &   & 76.57\ci{0.26}     & 90.03\ci{0.12}         \\
$\alpha$-TIM$_{\textrm{plc}}$*~\cite{alphaTIM}        & 70.95   & 89.56   \\
% \midrule
\rowcolor{LightCyan} $\alpha$-\ours & \tb{80.00} & 89.62 \\
\rowcolor{LightCyan} $\alpha$-\oursplc & 79.02 & \tb{89.80} \\

% \ours($\beta=0.8, k=20$)                & 80.00\ci{0.28}     & 89.72\ci{0.12}           \\ 
% PLC+\ours($\beta=0.8, k=20$)            & 79.02\ci{0.28}     & 89.62\ci{0.12}          \\ 
% \ours($\beta=0.9, k=10$)                & 76.81\ci{0.28}     & 89.64\ci{0.12}           \\ 
% PLC+\ours($\beta=0.9, k=10$)           & 77.03\ci{0.27}     & 89.80\ci{0.12}           \\
\bottomrule

\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:imbalanced_cub}
\end{table}
%------------------------------------------------------------------------------

%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
 \Th{Method}                                      & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}        \\ 

                                               & 1-shot              & 5-shot & 1-shot              & 5-shot           \\ \midrule
                                       \mc{5}{\Th{ResNet-18}}  \\ \midrule
                                       
%Entropy-min~\cite{entropy-min}              & - & - & - & -        \\
PT-MAP~\cite{pt_map}                           & 76.88    & 85.18   & 82.89    & 88.64          \\
LaplacianShot~\cite{laplacianshot}             & 70.24    & 82.10   & 77.28    & 86.22          \\
BD-CSPN~\cite{BDCSPN}                           & 69.36    & 82.06   & 76.36    & 86.18         \\
TIM~\cite{TIM}                                & 73.81    & 84.91   & 80.13    & 88.61       \\ 
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 69.33    & 84.53  & 76.36   & 88.33 \\
%\midrule
%$\alpha$-TIM*~\cite{alphaTIM}                &   & 67.15\ci{0.28}     & 82.53\ci{0.17}    & 74.34\ci{0.28}     & 86.68\ci{0.18} & - & - & - & -        \\
\rowcolor{LightCyan} \ours                                             & 76.37 & 84.85 & 82.68 & 88.60    \\  
\rowcolor{LightCyan} \oursplc                          & \tb{77.46} & \tb{85.47} & \tb{83.53} & \tb{89.06}       \\ 
\midrule
                                       \mc{5}{\Th{WRN-28-10}}  \\ \midrule
% Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & -     & - & -     & -       \\
% Baseline~\cite{closerlook}              &     &    & 62.2     & 81.9   & 63.5      & 83.8          \\
% Baseline++~\cite{closerlook}            &    &    & 64.5     & 82.1 & 68.0     & 84.2           \\
% Simpleshot~\cite{simpleshot}            &    &   & 66.2     & 82.4  & 69.6     & 84.7          \\
% \midrule
% MAML \cite{MAML}                         &  \multirow{11}*{WRN-28-10}  &  \multirow{11}*{Transdutive} & -     & -   & -     & -     \\
% Versa                                    &     &    & -     & -   & -     & -          \\
%Entropy-min \cite{entropy-min}         &  - & - & - & -           \\
PT-MAP~\cite{pt_map}                         &  80.35   & 87.37   & 84.84    & 89.86         \\
LaplacianShot~\cite{laplacianshot}             &  72.91    & 83.85   & 78.85    & 87.27         \\
BD-CSPN~\cite{BDCSPN}                   & 72.16   & 83.78   & 77.88   & 87.23       \\
TIM~\cite{TIM}                       &           77.78    & 87.43   & 82.28    & 89.84          \\ 
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 73.52    & 86.95   & 78.23    & 89.56 \\
%\midrule
\rowcolor{LightCyan} \ours                                             & 79.70 &  87.07 & 84.34 & 89.68   \\  
\rowcolor{LightCyan} \oursplc                           & \tb{81.05} & \tb{87.85} & \tb{85.34} & \tb{90.28}       \\ 

%$\alpha$-TIM*~\cite{alphaTIM}                &   & 70.32\ci{0.28}     & 84.91\ci{0.16}    & 75.97\ci{0.28}     & 87.75\ci{0.18}  & -    & -   & -    & -     \\
% \ours($\beta=0.8, k=20$)              &    &   & 72.54\ci{0.29}     & 84.17\ci{0.16}   & 78.90\ci{0.30}     & 87.63\ci{0.17}         \\  
% \ours($\beta=0.9, k=10$)               &    &   & 71.21\ci{0.29}     & 84.71\ci{0.16}   & 77.25\ci{0.29}     & 88.05\ci{0.17}        \\ 
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 71.55\ci{0.29}     & 84.78\ci{0.16}   & 78.66\ci{0.29}     & 88.01\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 71.48\ci{0.28}     & 85.71\ci{0.16}   & 77.90\ci{0.27}     & 88.67\ci{0.17}         \\  
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. All results are calculated using the the publicly available code provided from \cite{alphaTIM}. }
\label{tab:soa-balanced}
\end{table}
%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------


%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcc}
\toprule
\Th{Method}                            & \mc{2}{\Th{CUB}}        \\              
     & 1-shot              & 5-shot            \\ \midrule
% Protonet~\cite{prototypical}            & 64.51\ci{0.21}    & 86.91\ci{0.12}        \\
% Baseline~\cite{closerlook}               & 64.51\ci{0.21}    & 87.02\ci{0.11}         \\
% Baseline++~\cite{closerlook}            & 69.47\ci{0.21}    & 87.63\ci{0.11}         \\
% Simpleshot~\cite{simpleshot}            & 70.53\ci{0.20}    & 87.60\ci{0.11}        \\
% \midrule
%Entropy-min~\cite{entropy-min}          & -    & -         \\
PT-MAP~\cite{pt_map}                    & 86.05    & 91.28        \\
LaplacianShot~\cite{laplacianshot}      & 79.55    & 88.96         \\
BD-CSPN~\cite{BDCSPN}                   & 78.52   & 89.02        \\
TIM~\cite{TIM}                          & 82.87     & 91.58       \\
TIM$_{\textrm{plc}}$~\cite{TIM}                     & 77.69    & 91.17 \\
%\midrule
\rowcolor{LightCyan} \ours                                   & 85.88         & 91.35\\
\rowcolor{LightCyan} \oursplc                                & \tb{86.80}         & \tb{91.68} \\
% \midrule
% \ours($\beta=0.8, k=20$)                & 85.88\ci{0.24}    & 91.16\ci{0.10}        \\ 
% \ours($\beta=0.9, k=10$)                & 84.30\ci{0.23}    & 91.35\ci{0.10}        \\
% PLC+\ours($\beta=0.8, k=20$)            & 86.80\ci{0.23}    & 91.68\ci{0.10}        \\
% PLC+\ours($\beta=0.9, k=10$)            & 85.19\ci{0.23}    & 91.86\ci{0.10}         \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-balanced_cub}
\end{table}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

\subsubsection{Balanced transductive few-shot learning}
It can be seen from tables \ref{tab:soa-balanced} and \ref{tab:soa-balanced_cub} that \oursplc can outperform every other baseline with its closest competitor being PT-MAP~\cite{pt_map}. It should be noted that PT-MAP also uses \plc pre-processing meaning that our superiority is not based on the pre-processing. Comparing \ours against TIM it can be seen that we can significantly outperform them in all settings when \plc is used. Interestingly, TIM's performance is degraded through the use of \plc while \ours is improved which shows the robustness of our method. Even without \plc, \ours significantly outperforms TIM in the 1-shot setting by $\sim 2-4\%$ while performing on par or slightly worse on the 5-shot setting by $\sim 0.1-0.3\%$.



% \begin{comment}

\subsubsection{Balanced few-shot with different codebase}
Using code from \url{https://github.com/MichalisLazarou/iLPC}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \color{red}
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                               & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
                                        \mc{9}{\Th{WRN-28-10}}
%LR+ICI~\cite{lrici}                     & \multirow{4}*{ResNet-12}   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
% LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
%CAN+Top-\emph{k}~\cite{crossattention}  &     & 67.19\ci{0.55}      & 80.64\ci{0.35}      & 73.21\ci{0.58}      & 84.93 \ci{0.38}     & -                   & -                   & -                   & -                   \\
%DPGN~\cite{DPGN}                        &    & 67.77\ci{0.32}      & 84.60\ci{0.43}      & 72.45\ci{0.51}      & 87.24\ci{0.39}      & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
% EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}      & 76.53\ci{0.87}      & 87.32\ci{0.64}      & -                   & -                   & -                   & -                   \\
%MCT (instance)~\cite{mct}               &    & 78.55\ci{0.86}      & 86.03\ci{0.42}      & 82.32\ci{0.81}      & 87.36\ci{0.50}      & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
% MCT (Pair)~\cite{mct}                   & ResNet-12B   & 76.16\ci{0.89}      & 85.22\ci{0.42}      & 80.68\ci{0.89}      & 86.63\ci{0.89}      & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
% \tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55}  & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47}  & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\
\midrule
% PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
% Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}      & 73.34\ci{0.71}      & 85.50\ci{0.50}      & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}         & 70.74\ci{0.85}      & 84.34\ci{0.53}      & 78.50\ci{0.91}      & 88.36\ci{0.57}      & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}$\dagger$                     & 70.00\ci{0.60}      & 79.20\ci{0.40}      & 72.90\cip           & 82.80\cip           & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
% DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}      & -                   & -                   & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}              & 71.40\ci{0.50}      & 81.20\ci{0.40}      & 75.60\ci{0.6}       & 84.30\ci{0.4}       & -                   & -                   & -                   & -                   \\
%\tb{\ours (ours)}                       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
LaplacianShot~\cite{laplacianshot}  & 74.86\ci{0.19} & 84.13\ci{0.14} & 80.18\ci{0.21} & 87.56\ci{0.15} & - &- & -& -\\
PT+MAP~\cite{pt_map}                   &     & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
\ilpc~\cite{ilpc}          & 83.05\ci{0.79} & 88.82\ci{0.42} & 88.50\ci{0.75} & 92.46\ci{0.42} & 86.51\ci{0.75} & 90.60\ci{0.48} & 91.03\ci{0.63} & 94.11\ci{0.30}\\
EASE+SIAMESE~\cite{ease}          & 83.00\ci{0.21} & 88.92\ci{0.13} & \tb{88.96}\ci{0.23} & \tb{92.63}\ci{0.13} & \tb{87.60}\ci{0.23} & 90.60\ci{0.16} & \tb{91.68}\ci{0.19} & 94.12\ci{0.09}\\ \midrule
EASE+SIAMESE~\cite{ease}*          & 83.44\ci{0.77} & 88.66\ci{0.43} & 88.69\ci{0.73} & 92.47\ci{0.41} & 86.71\ci{0.77} & 90.28\ci{0.51} & 91.44\ci{0.63} & 93.85\ci{0.32} \\
EASE+SIAMESE$_\textrm{plc}$~\cite{ease}*          & 82.13\ci{0.81} & 87.34\ci{0.46}& 88.42\ci{0.73} & 92.19\ci{0.41} & 86.74\ci{0.78} & 90.22\ci{0.51} & 91.49\ci{0.63} & 93.32\ci{0.32} \\
%TIM \cite{TIM}      &     & 77.8\cip & 87.4\cip  & 82.1\cip & 89.8\cip & - & - & - & -\\
TIM* \cite{TIM}     &     & 77.65\ci{0.72} & 88.21\ci{40}  & 83.88\ci{0.74} & 91.89\ci{0.41} & 82.63\ci{0.70} & 90.28\ci{0.46} & 87.50\ci{0.62} & 93.59\ci{0.30}\\
TIM*$_{\textrm{plc}}$ \cite{TIM} &     & 75.77\ci{0.67} & 88.37\ci{0.40}  & 83.22\ci{0.70} & 92.13\ci{0.40} & 80.52\ci{0.70} & 90.25\ci{0.46} & 85.58\ci{0.61} & 93.48\ci{0.31}\\
% \ours ($\beta=0.8, K=20$)    &     & 80.83\ci{0.81} & 87.73\ci{0.42}  & 86.39\ci{0.77} & 91.67\ci{0.43} & 86.18\ci{0.74} & 90.14\ci{0.47} & 90.34\ci{0.68} & 93.47\ci{0.31}\\
% \ours($\beta=0.9, K=10$) &    & 79.68\ci{0.78} & 87.64\ci{0.42}  & 85.62\ci{0.76} & 91.74 & 84.99\ci{0.73} & 90.17\ci{0.46} & 89.64\ci{0.66} & 93.43\ci{0.31}\\
% \ours+PLC ($\beta=0.8, K=20$)    &    & 82.89\ci{0.72} & 89.03\ci{0.40}  & 88.07\ci{0.72} & 92.47\ci{0.40} & 86.81\ci{0.74} & 90.73\ci{0.46} & 91.11\ci{0.62} & 94.15\ci{0.29}\\
% i\ours+PLC ($\beta=0.8, K=20$)    &    & 82.83\ci{0.82} & -  & 88.09\ci{0.77} & - & 86.63\ci{0.79} & - & 91.05\ci{0.66} & -\\
% \ours+PLC($\beta=0.9, K=10$) &     & 81.52\ci{0.72} & 89.03\ci{0.40}  & 87.39\ci{0.71} & 92.49\ci{0.39} & 85.49\ci{0.72} & 90.76\ci{0.46} & 90.46\ci{0.60} & 94.08\ci{0.29}\\
\rowcolor{LightCyan} \ours            & 80.97\ci{0.82} & 87.75\ci{0.42}  & 86.51\ci{0.78} & 91.81\ci{0.43} & 86.25\ci{0.74} & 90.14\ci{0.47} & 90.53\ci{0.65} & 93.47\ci{0.30}\\
\rowcolor{LightCyan} \oursplc        & \tb{83.53}\ci{0.73} & \tb{89.06}\ci{0.40}  & 88.28\ci{0.73} &  92.61\ci{0.39} & 87.04\ci{0.74} & \tb{90.78}\ci{0.46} & 91.46\ci{0.60} & \tb{94.13}\ci{0.29} \\\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Balanced transductive inference state of the art}. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table*}
%---------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------}
%}

% \end{comment}

\subsection{Effect of unlabeled data}
%We argue that the slight performance deficit in the balanced 5-shot setting without \plc is simply a benchmarking limitation. 
We investigate the effect of unlabeled data comparing $\alpha$-\ours against $\alpha$-TIM. It can be seen from Table \ref{tab:trans-50q} that when using more unlabeled data, $M=250$, $\alpha$-\ours outperforms $\alpha$-TIM again in every setting. Impressively, the performance gap gets even larger than the standard setting of $M=75$. Particularly, the performance gap increases from $2.5\%$ to more than $4\%$ in the 1-shot \emph{mini}ImageNet and from $\sim0.3\%$ to more than $1\%$ in the 5-shot \emph{tiered}Imagenet. This can be attributed to the fact that $\alpha$-\ours captures the manifold structure while $\alpha$-TIM works in euclidean space. 


\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=67,
    % x dir=reverse,
	xlabel={shots},
	ylabel={mean accuracy},
    % legend style={at={(0.45,0.38)}},
	legend pos={north west},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[blue, mark=*] table[x=unlabeled, y=ours] \unlabeledone; \leg{$\alpha$-\ours}
\addplot[red, mark=*]  table[x=unlabeled,y=tim]  \unlabeledone; \leg{$\alpha$-TIM}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect of $\alpha$ for $\alpha$-\ours} on the 1-shot and 5-shot \emph{mini}ImageNet}
\label{fig:alpha_fig}
\end{figure}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lcccc}
\toprule
\Th{Method}   & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
           & 1-shot              & 5-shot              & 1-shot              & 5-shot\\ \midrule
                        \mc{5}{\Th{Imbalanced - ResNet-18}} \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}     & 69.53\ci{0.28}     & 83.73\ci{0.16}      & 76.07\ci{0.28}    & 87.13\ci{0.18}     \\
$\alpha$-\ours              & \tb{73.68}\ci{0.29} & \tb{83.97}\ci{0.16} &  \tb{80.43}\ci{0.29} & \tb{88.32}\ci{0.16}  \\ %\midrule
    %                    \mc{5}{\Th{Balanced - ResNet-18}} \\ \midrule
%TIM~\cite{TIM}     & 76.78\ci{0.24}     & 85.82\ci{0.12}     & 82.43\ci{0.24}    &  89.09\ci{0.13}     \\
%\ours              & 79.04\ci{0.26}      & 86.04 &  - & -  \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference, 250 queries in total}}
\label{tab:trans-50q}
\end{table}
%-----------------------------------------------------------------------------

\subsection{Other backbones}

\subsection{Ablation of $\alpha$}
We can see from Figure \ref{fig:alpha_fig} that $\alpha$ in both 1-shot and 5-shot 
\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=20,
    % x dir=reverse,
	xlabel={$\alpha$},
	ylabel={mean accuracy},
    legend style={at={(0.45,0.38)}},
	% legend pos={south east},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[violet, mark=*] table[x=alphavalues, y=oneshot] \alphagraph; \leg{1-shot}
\addplot[brown, mark=*]  table[x=alphavalues,y=fiveshot]  \alphagraph; \leg{5-shot}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect of $\alpha$ for $\alpha$-\ours} on the 1-shot and 5-shot \emph{mini}ImageNet}
\label{fig:alpha_fig}
\end{figure}
%------------------------------------------------------------------------------


\subsection{Robustness against imbalance}

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lcccc}
\toprule
\Th{Method}   & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
           & 1-shot              & 5-shot              & 1-shot              & 5-shot\\ \midrule
                        \mc{5}{\Th{Imbalanced - DenseNet-121}} \\ \midrule
$\alpha$-TIM~\cite{alphaTIM}     & 70.41  & 85.58 &  - & -     \\
$\alpha$-TIM$_{\textrm{plc}}$~\cite{alphaTIM}     & -  & - &  - & -     \\
$\alpha$-\ours              & 73.53      & 85.19 &  - & -  \\ 
$\alpha$-\oursplc              &-     & - &  - & -  \\ %\midrule
%                         \mc{5}{\Th{Balanced - DenseNet-121}} \\ \midrule
% TIM~\cite{TIM}     & -      & - &  - & -     \\
% \ours              & -      & - &  - & -  \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference, 50 queries per class}}
\label{tab:densenet}
\end{table}
%-----------------------------------------------------------------------------




% %------------------------------------------------------------------------------
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{5pt}
% \begin{tabular}{lccccc}
% \toprule
% \Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}       \\ 
%                                         &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                     \\ \midrule
% LR+ICI~\cite{lrici}*                    & ResNet-12A   & -     & -      & -      & -          \\
% CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12   & -     & -      & -      & -               \\
% DPGN~\cite{DPGN}                        & ResNet-12    & -     & -      & -      & -        \\
% MCT (instance)~\cite{mct}               & ResNet-12B   & -     & -      & -      & -          \\
% \midrule
% EP~\cite{embeddingpropagation}          & WRN-28-10    & -     & -      & -      & -                  \\
% SIB~\cite{SIB}$\dagger$                 & WRN-28-10    & -     & -      & -      & -                    \\
% SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & -     & -      & -      & -                     \\
% LaplacianShot~\cite{laplacianshot} & WRN-28-10 & -     & -      & -      & -  \\
% PT+MAP~\cite{pt_map}*                   & WRN-28-10   & -     & -      & -      & -    \\
%  \\ \bottomrule
% \end{tabular}
% \vspace{6pt}
% \caption{\emph{Transductive inference state of the art}. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
% \label{tab:soa-trans}
% \end{table}
% %------------------------------------------------------------------------------


% %------------------------------------------------------------------------------
% % \extdata{fig/data/sample}
% \begin{figure}
% % \extfig{pca}
% % {
% \begin{tikzpicture}
% \begin{axis}[
% 	width=\linewidth,
% 	height=0.5\linewidth,
% 	font=\small,
% 	ymin=67.2,
%     x dir=reverse,
% 	xlabel={shots},
% 	ylabel={mean accuracy},
% 	legend pos={south west},
% ]
% % \addplot [black, domain=0:3.5] {25*x^0.2};
% \addplot[blue, mark=*] table[x=shots,y=ours] \lowshot; \leg{$\alpha$-\ours (ours)}
% % \addplot[red, mark=*]  table[x=shots,y=tim]  \lowshot; \leg{$\alpha$-TIM}
% \end{axis}
% \end{tikzpicture}
% % }
% \caption{michalis}
% \label{fig:low_shot}
% \end{figure}
%------------------------------------------------------------------------------

==> tex/extra_experiments.tex <==
\clearpage


% PAGE NUMBER SET TO 1
\setcounter{page}{1}

% LINE NUMBER SET TO 1
\iccvrulercount=1

% START APPENDIX
\appendix

% COMMENT OUT \maketitle FROM main.tex FOR \maketitle TO WORK HERE
\maketitle
\subsection{Balanced transductive few-shot learning}
Using code from \url{https://github.com/MichalisLazarou/iLPC}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
LR+ICI~\cite{lrici}                     & \multirow{4}*{ResNet-12}   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
% LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
CAN+Top-\emph{k}~\cite{crossattention}  &     & 67.19\ci{0.55}      & 80.64\ci{0.35}      & 73.21\ci{0.58}      & 84.93 \ci{0.38}     & -                   & -                   & -                   & -                   \\
DPGN~\cite{DPGN}                        &    & 67.77\ci{0.32}      & 84.60\ci{0.43}      & 72.45\ci{0.51}      & 87.24\ci{0.39}      & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
% EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}      & 76.53\ci{0.87}      & 87.32\ci{0.64}      & -                   & -                   & -                   & -                   \\
MCT (instance)~\cite{mct}               &    & 78.55\ci{0.86}      & 86.03\ci{0.42}      & 82.32\ci{0.81}      & 87.36\ci{0.50}      & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
% MCT (Pair)~\cite{mct}                   & ResNet-12B   & 76.16\ci{0.89}      & 85.22\ci{0.42}      & 80.68\ci{0.89}      & 86.63\ci{0.89}      & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
% \tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55}  & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47}  & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\
\midrule
% PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
% Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}      & 73.34\ci{0.71}      & 85.50\ci{0.50}      & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}          & \multirow{14}*{WRN-28-10}    & 70.74\ci{0.85}      & 84.34\ci{0.53}      & 78.50\ci{0.91}      & 88.36\ci{0.57}      & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}$\dagger$                 &     & 70.00\ci{0.60}      & 79.20\ci{0.40}      & 72.90\cip           & 82.80\cip           & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
% DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}      & -                   & -                   & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}          &     & 71.40\ci{0.50}      & 81.20\ci{0.40}      & 75.60\ci{0.6}       & 84.30\ci{0.4}       & -                   & -                   & -                   & -                   \\
%\tb{\ours (ours)}                       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
LaplacianShot~\cite{laplacianshot} &  & 74.86\ci{0.19} & 84.13\ci{0.14} & 80.18\ci{0.21} & 87.56\ci{0.15} & - &- & -& -\\
PT+MAP~\cite{pt_map}                   &     & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
\ilpc~\cite{ilpc}      &     & 83.05\ci{0.79} & 88.82\ci{0.42} & 88.50\ci{0.75} & 92.46\ci{0.42} & 86.51\ci{0.75} & 90.60\ci{0.48} & 91.03\ci{0.63} & 94.11\ci{0.30}\\
EASE+SIAMESE~\cite{ease}      &     & 83.00\ci{0.21} & 88.92\ci{0.13} & 88.96\ci{0.23} & 92.63\ci{0.13} & 87.60\ci{0.23} & 90.60\ci{0.16} & 91.68\ci{0.19} & 94.12\ci{0.09}\\
TIM \cite{TIM}      &     & 77.8\cip & 87.4\cip  & 82.1\cip & 89.8\cip & - & - & - & -\\
TIM* \cite{TIM}     &     & 77.65\ci{0.72} & 88.21\ci{40}  & 83.88\ci{0.74} & 91.89\ci{0.41} & 82.63\ci{0.70} & 90.28\ci{0.46} & 87.50\ci{0.62} & 93.59\ci{0.30}\\
TIM*+PLC \cite{TIM} &     & 75.77\ci{0.67} & 88.37\ci{0.40}  & 83.22\ci{0.70} & 92.13\ci{0.40} & 80.52\ci{0.70} & 90.25\ci{0.46} & 85.58\ci{0.61} & 93.48\ci{0.31}\\
\ours ($\beta=0.8, K=20$)    &     & 80.83\ci{0.81} & 87.73\ci{0.42}  & 86.39\ci{0.77} & 91.67\ci{0.43} & 86.18\ci{0.74} & 90.14\ci{0.47} & 90.34\ci{0.68} & 93.47\ci{0.31}\\
\ours($\beta=0.9, K=10$) &    & 79.68\ci{0.78} & 87.64\ci{0.42}  & 85.62\ci{0.76} & 91.74 & 84.99\ci{0.73} & 90.17\ci{0.46} & 89.64\ci{0.66} & 93.43\ci{0.31}\\
\ours+PLC ($\beta=0.8, K=20$)    &    & 82.89\ci{0.72} & 89.03\ci{0.40}  & 88.07\ci{0.72} & 92.47\ci{0.40} & 86.81\ci{0.74} & 90.73\ci{0.46} & 91.11\ci{0.62} & 94.15\ci{0.29}\\
i\ours+PLC ($\beta=0.8, K=20$)    &    & 82.83\ci{0.82} & -  & 88.09\ci{0.77} & - & 86.63\ci{0.79} & - & 91.05\ci{0.66} & -\\
\ours+PLC($\beta=0.9, K=10$) &     & 81.52\ci{0.72} & 89.03\ci{0.40}  & 87.39\ci{0.71} & 92.49\ci{0.39} & 85.49\ci{0.72} & 90.76\ci{0.46} & 90.46\ci{0.60} & 94.08\ci{0.29}\\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{\emph{Balanced transductive inference state of the art}. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table*}
%---------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------



\section{Original tables transferred from main}
%-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Setting} & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}         \\ 
                                        &             &     & 1-shot              & 5-shot & 1-shot              & 5-shot               \\ \midrule
%Protonet~\cite{prototypical}            &  \multirow{4}*{ResNet-18}  &  \multirow{4}*{Inductive} & 53.4     & 74.2 &  -    & -       \\
%Baseline~\cite{closerlook}              &     &    & 56.0     & 78.9   & 63.5     & 83.8          \\
%Baseline++~\cite{closerlook}            &    &    & 60.4     & 79.7 & 68.0     & 84.2           \\
%Simpleshot~\cite{simpleshot}            &    &   & 63.0     & 80.1  & 69.6     & 84.7          \\
%\midrule
%MAML \cite{MAML}                         &  \multirow{11}*{ResNet-18}  &  \multirow{11}*{Transductive} & 47.6     & 64.5   & -     & -     \\
%Versa~\cite{versa}                                   &     &    & 47.8     & 61.9   & -     & -          \\
Entropy-min~\cite{entropy-min}           &    &    & 58.5     & 74.8    & 61.2     & 75.5           \\
LR+ICI~\cite{lrici}                      &    &    & 58.7     & 73.5    &  74.6    &   85.1        \\
PT-MAP~\cite{pt_map}                     &    &   & 60.1     & 67.1   & 64.1     & 70.0          \\
LaplacianShot~\cite{laplacianshot}       &    &   & 65.4     & 81.6   & 72.3     & 85.7          \\
BD-CSPN~\cite{BDCSPN}             &    &   & 67.0     & 80.2   & 74.1     & 84.8         \\
TIM~\cite{TIM}                           &    &   & 67.3     & 79.8   & 74.1     & 84.1        \\
$\alpha$-TIM~\cite{alphaTIM}             &    &   & 67.4     & 82.5    & 74.4    & 86.6        \\
$\alpha$-TIM*~\cite{alphaTIM}            &    &   & 67.15\ci{0.28}     & 82.53\ci{0.17}    & 74.34\ci{0.28}     & 86.68\ci{0.18}        \\
PLC+$\alpha$-TIM*~\cite{alphaTIM}            &    &   & 63.38\ci{0.24}     &   82.80\ci{0.17}   & 70.17\ci{0.26}     & 86.82\ci{0.18}      \\
%------------------------------------------------------OFFICIAL DATA WITH THE 2 VARIATIONS---------------------------------------------------------
% \ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.30}     & 82.12\ci{0.17}   & 77.28\ci{0.30}     & 86.59\ci{0.18}         \\  
% \ours($\beta=0.9, k=10$)               &    &   & 68.44\ci{0.29}     & 82.41\ci{0.17}   & 75.73\ci{0.29}     & 87.02\ci{0.18}         \\ 
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 70.03\ci{0.29}     & 82.75\ci{0.17}   & 76.59\ci{0.29}      & 86.72\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 68.99\ci{0.29}     & 83.27\ci{0.17}   & 75.75\ci{0.28}    & 87.28\ci{0.17}         \\
%--------------------------------------------------------------------------------------------------------------------------------------------------
$\alpha$-\ours                               &    &   & \tb{70.03}\ci{0.30}     & 82.41\ci{0.17}   & \tb{77.28}\ci{0.30}     & 87.02\ci{0.18}         \\  
PLC+$\alpha$-\ours                            &    &   &  \tb{70.03}\ci{0.29}     & \tb{83.27}\ci{0.17}   & 76.59\ci{0.29}   & \tb{87.28}\ci{0.17}         \\ 
\midrule
% Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & -     & - & -     & -       \\
% Baseline~\cite{closerlook}              &     &    & 62.2     & 81.9   & 63.5      & 83.8          \\
% Baseline++~\cite{closerlook}            &    &    & 64.5     & 82.1 & 68.0     & 84.2           \\
% Simpleshot~\cite{simpleshot}            &    &   & 66.2     & 82.4  & 69.6     & 84.7          \\
% \midrule
% MAML \cite{MAML}                         &  \multirow{11}*{WRN-28-10}  &  \multirow{11}*{Transdutive} & -     & -   & -     & -     \\
% Versa                                    &     &    & -     & -   & -     & -          \\
Entropy-min \cite{entropy-min}          & \multirow{12}*{WRN-28-10}  &  \multirow{12}*{Transductive}& 60.4    & 76.2 & 62.9     & 77.3           \\
% LR+ICI~\cite{lrici}                      &    &    & -     & - & -     & -           \\
PT-MAP~\cite{pt_map}                     &    &   & 60.6     & 66.8   & 65.1     & 71.0         \\
LaplacianShot~\cite{laplacianshot}       &    &   & 68.1     & 83.2   & 73.5     & 86.8         \\
BD-CSPN~\cite{BDCSPN}             &    &   & 70.4     & 82.3   &  75.4    & 85.9         \\
TIM~\cite{TIM}                           &    &   & 69.8     & 81.6    & 75.8    & 85.4        \\
$\alpha$-TIM~\cite{alphaTIM}             &    &   & 69.8     & 84.8     & 76.0   & 87.8        \\
$\alpha$-TIM*~\cite{alphaTIM}            &    &   & 70.32\ci{0.28}     & 84.91\ci{0.16}    & 75.97\ci{0.28}     & 87.75\ci{0.18}        \\
PLC+$\alpha$-TIM*~\cite{alphaTIM}            &    &   & 66.50\ci{0.24}     & 85.12\ci{0.16}    & 71.97\ci{0.25}     &  88.28\ci{0.16}      \\
% \ours($\beta=0.8, k=20$)              &    &   & 72.54\ci{0.29}     & 84.17\ci{0.16}   & 78.90\ci{0.30}     & 87.63\ci{0.17}         \\  
% \ours($\beta=0.9, k=10$)               &    &   & 71.21\ci{0.29}     & 84.71\ci{0.16}   & 77.25\ci{0.29}     & 88.05\ci{0.17}        \\ 
% PLC+\ours($\beta=0.8, k=20$)              &    &   & 71.55\ci{0.29}     & 84.78\ci{0.16}   & 78.66\ci{0.29}     & 88.01\ci{0.17}         \\
% PLC+\ours($\beta=0.9, k=10$)             &    &   & 71.48\ci{0.28}     & 85.71\ci{0.16}   & 77.90\ci{0.27}     & 88.67\ci{0.17}         \\  
$\alpha$-\ours                        &    &   & \tb{72.54}\ci{0.29}     & 84.71\ci{0.16}   & \tb{78.90}\ci{0.30}     & 88.05\ci{0.17}        \\  
PLC+$\alpha$-\ours                       &    &   & 71.55\ci{0.29}     & \tb{85.71}\ci{0.16}   & 78.66\ci{0.29}     & \tb{88.67}\ci{0.17}        \\

\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table*}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------


%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Setting} & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}}         \\ 
                                        &             &     & 1-shot              & 5-shot & 1-shot              & 5-shot               \\ \midrule
Protonet~\cite{prototypical}            &  \multirow{4}*{ResNet-18}  &  \multirow{4}*{Inductive} & 56.10\ci{0.20}    & 78.72\ci{0.15}   & 63.28\ci{0.23}    & 84.10\ci{0.16}         \\
Baseline~\cite{closerlook}              &     &    & 56.10\ci{0.20}    & 78.80\ci{0.14}   & 63.28\ci{0.23}    & 84.12\ci{0.16}         \\
Baseline++~\cite{closerlook}            &    &    & 60.22\ci{0.20}    & 79.72\ci{0.14}   & 68.06\ci{0.22}    & 84.50\ci{0.15}         \\
Simpleshot~\cite{simpleshot}            &    &   & 63.00\ci{0.20}    & 80.09\ci{0.14}   & 69.72\ci{0.22}    & 84.87\ci{0.15}         \\
\midrule
Entropy-min~\cite{entropy-min}           &  \multirow{11}*{ResNet-18}  &  \multirow{11}*{Transductive} & -    & -   & -    & -         \\
PT-MAP~\cite{pt_map}                     &    &   & 76.88\ci{0.27}    & 85.18\ci{0.14}   & 82.89\ci{0.26}    & 88.64\ci{0.15}         \\
LaplacianShot~\cite{laplacianshot}       &    &   & 70.24\ci{0.23}    & 82.10\ci{0.14}   & 77.28\ci{0.24}    & 86.22\ci{0.16}         \\
BD-CSPN~\cite{BDCSPN}             &    &   & 69.36\ci{0.23}    & 82.06\ci{0.14}   & 76.36\ci{0.24}    & 86.18\ci{0.16}         \\
TIM~\cite{TIM}                           &    &   & 73.81\ci{0.25}    & 84.91\ci{0.15}   & 80.13\ci{0.25}    & 88.61\ci{0.15}         \\
PLC+TIM*~\cite{TIM}            &    &   & 69.33\ci{0.23}    & 84.53\ci{0.14}   & 76.36\ci{0.24}    & 88.33\ci{0.15}         \\
\ours($\beta=0.8, k=20$)              &    &   & 76.37\ci{0.28}    & 84.85\ci{0.15}   &  82.68\ci{0.27}    & 88.29\ci{0.16}         \\ 
\ours($\beta=0.9, k=10$)               &    &   & 74.87\ci{0.27}    & 84.80\ci{0.15}   & 81.70\ci{0.26}    & 88.60\ci{0.15}         \\
PLC+\ours($\beta=0.8, k=20$)              &    &   & 77.46\ci{0.27}    & 85.25\ci{0.14}   & 83.53\ci{0.26}    & 88.85\ci{0.15}         \\
PLC+\ours($\beta=0.9, k=10$)             &    &   & 75.84\ci{0.26}    & \tb{85.47}\ci{0.14}   & 82.17\ci{0.25}    & 89.06\ci{0.15}         \\
\midrule
Protonet~\cite{prototypical}            &  \multirow{4}*{WRN-28-10}  &  \multirow{4}*{Inductive} & 60.87\ci{0.20}     & 81.52\ci{0.14} & 64.59\ci{0.23}     & 84.95\ci{0.16}       \\
Baseline~\cite{closerlook}              &     &    & 60.87\ci{0.20}    & 81.61\ci{0.14}   & 64.59\ci{0.23}    & 84.97\ci{0.16}         \\
Baseline++~\cite{closerlook}            &    &    & 63.10\ci{0.20}    & 82.02\ci{0.14}   & 68.58\ci{0.22}    & 85.43\ci{0.15}         \\
Simpleshot~\cite{simpleshot}            &    &   &  65.76\ci{0.20}    & 82.27\ci{0.14}   & 70.77\ci{0.22}    & 85.81\ci{0.15}         \\
\midrule
Entropy-min \cite{entropy-min}          & \multirow{12}*{WRN-28-10}  &  \multirow{12}*{Transductive} & -    & -   & -    & -         \\
PT-MAP~\cite{pt_map}                     &    &   & 80.35\ci{0.25}    & 87.37\ci{0.13}   & 84.84\ci{0.25}    & 89.86\ci{0.15}         \\
LaplacianShot~\cite{laplacianshot}       &    &   & 72.91\ci{0.23}    & 83.85\ci{0.14}   & 78.85\ci{0.24}    & 87.27\ci{0.15}         \\ 
BD-CSPN~\cite{BDCSPN}             &    &   & 72.16\ci{0.22}    & 83.78\ci{0.14}   & 77.88\ci{0.24}    & 87.23\ci{0.15}         \\
TIM~\cite{TIM}                           &    &  & 77.78\ci{0.24}    & 87.43\ci{0.13}   & 82.28\ci{0.24}    & 89.84\ci{0.15}         \\
PLC+TIM*~\cite{TIM}            &    &  & 73.52\ci{0.22}    & 86.95\ci{0.95}   & 78.23\ci{0.24}    & 89.56\ci{0.14}         \\
\ours($\beta=0.8, k=20$)              &    &   & 79.70\ci{0.26}    & 86.91\ci{0.13}   & 84.34\ci{0.26}    & 89.36\ci{0.15}         \\ 
\ours($\beta=0.9, k=10$)               &    &   & 78.27\ci{0.26}    & 87.07\ci{0.13}   & 83.44\ci{0.25}    & 89.68\ci{0.15}         \\
PLC+\ours($\beta=0.8, k=20$)              &    &   & 81.04\ci{0.26}    & 87.61\ci{0.13}   & 85.34\ci{0.25}    & 90.06\ci{0.15}         \\
PLC+\ours($\beta=0.9, k=10$)             &    &   & 79.58\ci{0.25}    & 87.85\ci{0.13}   & 84.21\ci{0.24}    & 90.28\ci{0.14}         \\  
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table*}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{table*}
\small
\centering
% \begin{adjustbox}{width=1\coluwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Setting} & \mc{2}{\Th{CUB}}        \\              
    &             &     & 1-shot              & 5-shot            \\ \midrule
Protonet~\cite{prototypical}            &  \multirow{4}*{ResNet-18}  &  \multirow{4}*{Inductive} & 64.51\ci{0.21}    & 86.91\ci{0.12}        \\
Baseline~\cite{closerlook}              &     &    & 64.51\ci{0.21}    & 87.02\ci{0.11}         \\
Baseline++~\cite{closerlook}            &    &    & 69.47\ci{0.21}    & 87.63\ci{0.11}         \\
Simpleshot~\cite{simpleshot}            &    &   & 70.53\ci{0.20}    & 87.60\ci{0.11}        \\
\midrule
Entropy-min~\cite{entropy-min}          &  \multirow{8}*{ResNet-18}  &  \multirow{11}*{Transductive} & -    & -         \\
PT-MAP~\cite{pt_map}                    &    &   & 86.05\ci{0.23}    & 91.28\ci{0.11}         \\
LaplacianShot~\cite{laplacianshot}      &    &   & 79.55\ci{0.22}    & 88.96\ci{0.11}         \\
BD-CSPN~\cite{BDCSPN}                   &    &   & 78.52\ci{0.22}    & 89.02\ci{0.11}         \\
TIM~\cite{TIM}                          &    &   & 82.87\ci{0.22}     & 91.58\ci{0.10}       \\
PLC+TIM*~\cite{TIM}                     &    &   & 77.69\ci{0.22}    & 91.17\ci{0.10} \\
\ours($\beta=0.8, k=20$)                &    &   & 85.88\ci{0.24}    & 91.16\ci{0.10}        \\ 
\ours($\beta=0.9, k=10$)                &    &   & 84.30\ci{0.23}    & 91.35\ci{0.10}        \\
PLC+\ours($\beta=0.8, k=20$)            &    &   & 86.80\ci{0.23}    & 91.68\ci{0.10}        \\
PLC+\ours($\beta=0.9, k=10$)            &    &   & 85.19\ci{0.23}    & 91.86\ci{0.10}         \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Balanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans_cub}
\end{table*}
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
% \small
\centering
% \begin{adjustbox}{width=1\columnwidth}
\setlength\tabcolsep{5pt}
\begin{tabular}{lcccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Setting} & \mc{2}{\Th{CUB}}       \\ 
                                        &             &     & 1-shot              & 5-shot         \\ \midrule
Baseline~\cite{closerlook}              &  \multirow{3}*{ResNet-18}  &  \multirow{3}*{Inductive}    & 64.6     & 86.9          \\
Baseline++~\cite{closerlook}            &    &    & 69.4     & 87.5            \\
Simpleshot~\cite{simpleshot}            &    &   & 70.6     & 87.5          \\
\midrule
PT-MAP~\cite{pt_map}                     &  \multirow{11}*{ResNet-18}  &  \multirow{11}*{Transductive} & 65.1     & 71.3      \\
Entropy-min~\cite{entropy-min}           &    &   & 67.5     & 82.9          \\
LaplacianShot~\cite{laplacianshot}       &    &   & 73.7     & 87.7           \\
BD-CSPN~\cite{BDCSPN}                   &    &   & 74.5     & 87.1           \\
TIM~\cite{TIM}                           &    &   & 74.8     & 86.9        \\
$\alpha$-TIM~\cite{alphaTIM}             &    &   & 75.7     & 89.8       \\
*$\alpha$-TIM~\cite{alphaTIM}            &    &   & 76.57\ci{0.26}     & 90.03\ci{0.12}         \\
PLC+$\alpha$-TIM*~\cite{alphaTIM}        &    &   & 70.95\ci{0.23}    & 89.56\ci{0.12}   \\
\ours($\beta=0.8, k=20$)                &    &   & 80.00\ci{0.28}     & 89.72\ci{0.12}           \\ 
PLC+\ours($\beta=0.8, k=20$)            &    &   & 79.02\ci{0.28}     & 89.62\ci{0.12}          \\ 
\ours($\beta=0.9, k=10$)                &    &   & 76.81\ci{0.28}     & 89.64\ci{0.12}           \\ 
PLC+\ours($\beta=0.9, k=10$)            &    &   & 77.03\ci{0.27}     & 89.80\ci{0.12}           \\\bottomrule

\end{tabular}
% \end{adjustbox}
\vspace{6pt}
\caption{\emph{Imbalanced transductive inference experimental comparisons with state of the art}. The results are reported as provided from \cite{alphaTIM}. *: our reproduction with official code using the publicly available code provided from \cite{alphaTIM}. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table}
%------------------------------------------------------------------------------



\subsection{Low-shot learning}
\label{sec:low_shot}

In this section we compare the robustness of \ours TIM with respect to the number of labeled support images per class. We focus on the balanced setting since the $\alpha$ values are only defined for the 1-shot and 5-shot setting from \cite{alphaTIM}.

%------------------------------------------------------------------------------
\extdata{fig/data/sample}
\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	ymin=67.2,
    x dir=reverse,
	xlabel={shots},
	ylabel={mean accuracy},
	legend pos={south west},
]
% \addplot [black, domain=0:3.5] {25*x^0.2};
\addplot[blue, mark=*] table[x=shots,y=ours] \lowshot; \leg{$\alpha$-\ours (ours)}
\addplot[red, mark=*]  table[x=shots,y=tim]  \lowshot; \leg{$\alpha$-TIM}
\end{axis}
\end{tikzpicture}
}
\caption{\emph{Effect on decreasing the number on shots on $\alpha$-\ours and $\alpha$-TIM} on the imbalanced few-shot learning with \emph{mini}ImageNet, $\alpha=2$}
\label{fig:low_shot}
\end{figure}
%------------------------------------------------------------------------------

% %------------------------------------------------------------------------------
% \extdata{fig/data/sample}
% \begin{figure}
% \extfig{pca}
% {
% \begin{tikzpicture}
% \begin{axis}[
% 	width=\linewidth,
% 	height=0.5\linewidth,
% 	font=\small,
% 	ymin=67.2,
%     x dir=reverse,
% 	xlabel={shots},
% 	ylabel={mean accuracy},
% 	legend pos={south west},
% ]
% % \addplot [black, domain=0:3.5] {25*x^0.2};
% \addplot[blue, mark=*] table[x=shots,y=ours] \lowshotbal; \leg{\ours (ours)}
% \addplot[red, mark=*]  table[x=shots,y=tim]  \lowshotbal; \leg{TIM}
% \end{axis}
% \end{tikzpicture}
% }
% \caption{\emph{Effect on decreasing the number on shots on \ours and TIM} on the imbalanced few-shot learning with \emph{mini}ImageNet, $\alpha=2$}
% \label{fig:low_shot}
% \end{figure}
% %------------------------------------------------------------------------------



==> tex/intro-1.tex <==
\section{Introduction}
\label{sec:intro}

%---------------------------------------------------------------------------------------------------
\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{fig/ICCV23_idea.pdf}
% \fig{ICCV23_idea}
\vspace{0pt}
\caption{\emph{Overview of our method}}
\label{fig:overview}
\end{figure}
%------------------------------------------------------------------------------------------------

Deep learning has transformed computer vision by continuously improving the state of the art in many computer vision applications such as segmentation, detection and classification. However one of its fundamental limitations is its reliance on large labeled datasets. Labeled datasets can be very tedious to create because of the human labour required for labeling them and the difficulty in obtaining data in certain applications where the data can be scarce for example in rare animal species classification \cite{bertinetto}.

The few-shot learning paradigm has attracted significant interest in recent years from the research community since it investigates the research question of how to make deep learning models acquire knowledge from limited data~\cite{matchingNets, prototypical, MAML}.  Various different methodologies have been proposed to address few-shot learning such as \emph{meta-learning}~\cite{prototypical, MAML, siamese}, \emph{transfer learning}~\cite{rfs, manifoldmixup, denseclassification}, synthetic data generation generation~\cite{AFHN, VIFSL, TFH}. However, the vast majority of these methods focus on the inductive few-shot learning paradigm, where the assumption is that during inference every query example is classified independently of the other.

Recent studies explored transductive few-shot learning, where all test examples are available during test time and can be exploited together, showing remarkable performance improvements \cite{ilpc, pt_map, lrici, ease, oblique_manifold}.  Current state of the art methods exploit the test example at inference time through numerous ways, a common way is by exploiting the manifold structure of the data through label propagation \cite{ilpc} or by using the properties of oblique manifold \cite{oblique_manifold}. Another direction focuses on utilizing the test samples to improve the class centroids such as by adapting the class centroids through specialized loss functions \cite{TIM}, using soft K-means \cite{pt_map} and by minimizing the cross-class and intra-class variance\cite{BDCSPN}. % It has also been shown that selecting iteratively the most confident pseudo-labeled examples to augment the support set is another effective way to boost the performance \cite{lrici, ilpc}.

While transductive few-shot learning methods have shown impressive performance with respect to their inductive counterparts, it has been argued in \cite{alphaTIM} that transductive few-shot learning benchmarks are not reliable because they use perfectly class-balanced tasks. Several state of the art methods make this assumption and utilize class balancing techniques \cite{ilpc, ease, pt_map, TIM} to improve their performance. However, this is unrealistic and as a way to address this  \cite{alphaTIM} proposed a novel imbalanced transductive few-shot learning setting comparing numerous state of the art methods fairly and showing that their performances dramatically decrease.

% our idea.
%In this work we focus on the imbalanced transductive few-shot learning setting \cite{alphaTIM} and propose a novel algorithm, named \emph{Manifold similarity centroids} (MSC) that provides state of the art performance. Also, we show that our algorithm can perform on par with state of the art approaches on the balanced transductive few-shot learning setting as well. Particularly, our algorithm combines the merits of the aforementioned two main lines of research, exploiting the test examples to obtain more representative class centroids by exploiting the manifold structure of the data. 

In this work we focus on the imbalanced transductive few-shot learning setting \cite{alphaTIM} and propose a novel algorithm, named \emph{Manifold similarity centroids} that combines the merits of class centroid approaches as well as exploiting the manifold of the data. More specifically we initialize the class centroids from the labeled support examples and we leverage the underlying data manifold by propagating labels from the class centroids to all data through the use of an adaptive $k$-nearest neighbour graph \cite{semilpavrithis}. We utilize the manifold similarities of all the data obtained after the label propagation to calculate class probability distribution for both support and query sets. Using the differentiable loss function proposed in \cite{TIM} and \cite{alphaTIM} we update both the class centroids as well as the constructed graph's parameters. Finally we iterate the procedure from constructing a graph to obtaining probabilities optimizing the manifold centroids and the constructed graph's parameters until convergence. Our algorithm outperforms other state of the art methods in the imbalanced transductive few-shot learning settingg.

We summarize our contributions below:
\begin{itemize}
    \item We are the first, to the best of our knowledge, to calculate class centroids through manifold class similarity. by utilizing a $k$-nearest neighbour graph.
    \item We are the first, to the best of our knowledge, to propose to optimize both the class centroids along with the manifold graph structure through a differentiable loss function.
    \item We achieve new state of the art performances in the majority of the imbalanced transductive few-shot learning settings under multiple benchmark datasets and backbones, surpassing by as much as $3.5\%$ the previous state of the art in the 1-shot setting.
    \item We show that our method can also perform on par or even surpass many state of the art methods in the standard balanced transductive few-shot learning setting.
    % \item \alert{We show the robustness of leveraging manifold similarity compared to cosine distance in other few-shot learning settings.}
\end{itemize}

==> tex/method-1.tex <==
\section{Method}
\label{sec:method}

\subsection{Problem formulation}
\label{sec:problem_defs}
We assume access to backbone network, $f_{\theta}$, that has been pre-trained on a dataset $D_{\base} = \{(x_i, y_i)\}_{i=1}^B$ of total size $B$ where each image $x_i$ has a corresponding label $y_i$ from one of the classes in $C_{\base}$.

At inference stage we assume access to a dataset $D_{\novel}$ consisting of images with corresponding labels from $C_{\novel}$ where $C_{\novel} \cap C_{\base} = \emptyset$. We sample N-way K-shot tasks consisting of a labeled support set, $S = \{(X_S, Y_S)\}$, that contains examples from N different classes from $C_{\novel}$ with K examples per class with the total number of examples in the support set denoted as $L=NK$. In the transductive few-shot learning setting, a task also consists of a query set, $Q = \{(X_Q, Y_Q)\}$ where the query examples are sampled from exactly the same $N$ classes as the support set $S$. The total number of queries is $M$ and in the balanced setting we have the added information that there are $\frac{M}{N}$ query examples per class. $X_S$ and $X_Q$ denote the images that belong to $S$ and $Q$ respectively while $Y_S$ and $Y_Q$ denote the labels that correspond to $X_S$ and $X_Q$ respectively.%We denote the labels corresponding to $S$ and $Q$ as $Y_{S}$ and $Y_Q$ respectively.

\subsection{Feature extraction}
\label{sec:embeddings}

For every task we assume access to a support set $S = \{(x_i, y_i)\}_{i=1}^L$, a query set $Q = \{(x_i, y_i)\}_{i=1}^M$ and the pre-trained backbone $f_{\theta}$. We embedding all images in $S$ and $Q$ into the vector set $V = \{(\vv_i)\}_{i=1}^{T}$, where $T=L+M$ and the first $L$ examples correspond to the images from $S$ and $\vv_i = f_{\theta}(x_i)$. We experiment with two commonly used pre-processing techniques to pre-process each vector in $V$, $\ell_2$-normalization and the pre-processing used in \cite{pt_map, ilpc} that we will refer to as \plc. $\ell_2$-normalization is simply defined as $\vv_i = \frac{\vv_i}{||\vv_i||_2}$ for every $\vv_i \in V$. \plc performs elementwise power transform to the $0.5$ for all $\vv_i \in V$  followed by $\ell_2$-normalization and centering using the mean of all vectors in $V$.

% he first technique is simply $\ell_2$-normalization of all vectors in $V$ while the for the second we follow% defined as $\vv_i = \frac{\vv_i}{||\vv_i||_2}$ for vector $\vv_i \in V$ and the second one is the pre-processing used 
% \cite{pt_map, ilpc} and perform elementwise power transform to the $0.5$ for all $\vv_i \in V$  followed by $\ell_2$-normalization and centering using the mean of all vectors in $V$. We will refer to the second pre-processing technique as \plc.


\subsection{Class centroids}
\label{sec:centroids}
Following \cite{prototypical}, we calculate the class centroids of every class represented in the support set $S$, where the class centroid of class $j$ is essentially the mean vector of all the support vectors belonging to class $j$ defined as:
\begin{equation}
    \cc_j \defn \frac{1}{|S_j|} \sum_{\vv_i \in S_j}(\vv_i) %\big\displaystyle\sum_{\vv_i \in S}(\vv_i)
\end{equation}
where $S_j$ denotes all vectors belonging to class $k$. We denote the set of all class centroids as $\cC =\{\cc_1,\dots,\cc_j\}_{j=1}^N$.

\subsection{Nearest neighbour graph construction}
\label{sec:graph_contruction}
Following \cite{semilpavrithis, ilpc}, we construct a $k$-nearest neighbour graph using all the class centroids in $\cC$ along with all vectors in $V$. We denote the set of $V \cup \cC = U$, where $U = \{\uu_i,\dots, \uu_H\}_{h=1}^H$ and $H=T+N$. The graph is represented by an \emph{affinity matrix} $A$ of size $H \times H$ defined as:

\begin{equation}
	A_{ij} \defn
	\begin{cases}
		\mathrm{exp}(-\frac{||\uu_i-\uu_j||_2^2}{g_{ij}\sigma}), & \mif i \ne j \wedge \uu_i \in \NN_k(\uu_j) \\
		0,                           & (\uu_i, \uu_j) \in \cC \\
  		0,                           & \other
	\end{cases}
\label{eq:affinity}
\end{equation}


where $g_{ij}$ represents a unique pairwise scaling factor for every pair $||\uu_i-\uu_j||_2^2$ while $\sigma$ represents the standard deviation of $||\uu_i-\uu_j||_2^2$ for all pairs of $(\uu_i, \uu_j) \in U$ and $\NN_k(\uu_j)$ represents the $k$-nearest neighbours of $\uu_j$ from set $U$. We denote the set $\cG \in g_{ij}$ as the set of all scaling factors. We obtain the \emph{adjacency matrix} defined as $W \defn \frac{1}{2} (A + A\tran)$ before symmetrically normalize it:
\begin{equation}
    \cW \defn D^{-1/2} W D^{-1/2},
\label{eq:adj}
\end{equation}
where $D = \diag(W \vone_T)$ is the $H \times H$ degree matrix of $W$.
\subsection{Label Propagation}
\label{sec:lp}
Following~\cite{ZBL+03}, we define the \emph{label matrix} of size $H \times N$ as:
\begin{equation}
 Y_{ij} \defn
	\begin{cases}
		1, & \mif i \le N \wedge y_i = j \\
		0, & \other
	 \end{cases}
\label{eq:label}
\end{equation}
where $i \in H$ and $j \in N$. Matrix $Y$ has one column per class and one row per example, which is an one-hot encoded label for every class centroid in $C$ and a zero vector for both $S$ and $Q$. Leveraging the constructed graph structure we carry out label propagation by solving: 

\begin{equation}
    Z \defn (I-\cB \circ \cW)^{-1} Y,
\label{eq:lp}
\end{equation}
where $\cB$ is an $H \times H$ matrix of scalar values, $\cB_{i,j} \in (0,1]$ for $i \in H$, $j \in H$ and $\circ$ represents the Hadamard multiplication of $\cB$ and $\cW$. The resulting \emph{manifold class similarity matrix}, $Z$, provides information of how similar example $x_i$ is to each of the N support classes through the manifold similarity vector $z_i$ that is the $i^{th}$ row of $Z$. By using the softmax function we calculate the probability matrix $P$ where every row $i$ provides the probability vector $p_i$:

\begin{equation}
    p_{i} \defn \frac{\exp(\tau z_{i})}{\sum_{j=1}^N \exp(\tau z_{ij})},
\label{eq:softmax}
\end{equation}
where $\tau$ is a positive hyperparameter analogous to the scaling temperature used in softmax-based classifiers. The rows of $P$ from $\{1, \cdots, N\}$, $\{N, \cdots,N+L\}$ and $\{N+L, \cdots,N+L+M\}$ define three submatrices that hold the probability distributions of $\cC$, $S$ and $Q$ respectively. We denote these submatrices as $P^{\cC}$, $P^S$ and $P^Q$ and their corresponding row vectors as $p^c$, $p^s$ and $p^q$.


%$P$ is made up of three submatrices: centroid probability matrix $P^{\cC} \in P[:N]$, support probability matrix $P^S\in P[N:N+L]$ and query probability matrix $P^Q\in P[N+L:]$ where each each submatrix holds the probability distribution regarding $\cC$, $S$ and $Q$ respectively.

\subsection{Mutual-information maximization}
We define the set of learnable manifold parameters as $\Phi = \{\cC, \cG, \cB \}$ that are updated iteratively through the minimization of a mutual information loss proposed \cite{TIM, alphaTIM}.
\label{sec:TIM}
\subsubsection{Balanced}
Following \cite{TIM}, we optimize parameters $\Phi$ through the use of the proposed loss function composed of the following three terms:
% \begin{equation}
% \begin{split}
%     L_{ce}(X_S;Y_S) & \defn -\frac{1}{NK}\sum_{i\in S}\sum_{j=1}^Ny_{ij}\log(p^s_{ij})\\
%     \mathcal{H}(Y_Q|X_Q) & \defn -\frac{1}{M}\sum_{i\in Q}\sum_{j=1}^Np^q_{ij}\log(p^q_{ij})\\
%     \mathcal{H}(Y_Q) & \defn -\sum_{j=1}^N\hat{p}^q_j\log(\hat{p}^q_{j})\\
% \label{eq:TIM_equations}
% \end{split}
% \end{equation}

\begin{equation}
    L_{ce}(X_S;Y_S) \defn -\frac{1}{NK}\sum_{i\in S}\sum_{j=1}^Ny_{ij}\log(p^s_{ij})\\
\label{eq:ce}
\end{equation}

\begin{equation}
    \mathcal{H}(Y_Q|X_Q) \defn -\frac{1}{M}\sum_{i\in Q}\sum_{j=1}^Np^q_{ij}\log(p^q_{ij})\\
\label{eq:conditional_entropy}
\end{equation}

\begin{equation}
    \mathcal{H}(Y_Q) \defn -\sum_{j=1}^N\hat{p}^q_j\log(\hat{p}^q_{j})\\
\label{eq:label_entropy}
\end{equation}
where $y_{ij}$ represents the $j^{th}$ component of the one-hot label $y_i$ of the $i^{th}$ support example while $p^s_{ij}$ and $p^q_{ij}$ represent the $h^{th}$ component of the probability row vector of the $i^{th}$ row of $P^S$ and $P^Q$ respectively. The term $\hat{p}^q_j = \frac{1}{M}\sum_{i\in Q}p^q_{ij}$ is the marginal distribution over query labels. $L_{ce}(X_S;Y_S)$ is the cross entropy loss on the support set, $S$, $\mathcal{H}(Y_Q|X_Q)$ is the conditional entropy aiming at minimizing the uncertainty of the predicted probability distributions of the query set, $Q$, and $\mathcal{H}(Y_Q)$ is the label-marginal entropy term. The weighted mutual information is defined as:
\begin{equation}
    \mathcal{I}(X_Q; Y_Q) \defn \lambda_1\mathcal{H}(Y_Q) - \lambda_2\mathcal{H}(Y_Q|X_Q)
\end{equation}
where $\lambda_1$ and $\lambda-2$ are scalar hyperparameters. The final loss function minimized with respect to $\Phi$ is defined as:
\begin{equation}
    L_{bal}(S;Q) \defn \lambda_3 L_{ce}(X_S; Y_S) -\mathcal{I}(X_Q; Y_Q)%+  \lambda_2\mathcal{H}(Y_Q|X_Q) -\lambda_3\mathcal{H}(Y_Q)%-\lambda_1\frac{1}{|S|}\sum_{i\in S}\sum_{k=1}^Ky_{ik}\log(p_{ik}) -\big\displaystyle(-\sum_
\label{eq:balanced}
\end{equation}
where $\lambda_3$ is another scalar hyperparameters.

\subsubsection{Imbalanced}
As it was discussed in \ref{sec:cls_bal}, it was argued in \cite{alphaTIM} that minimizing the label-marginal entropy term $\mathcal{H}(Y_Q)$ encourages class-balanced solutions since it has been shown that is is equivalent to minimizing the the KL divergence between predicted probability distribution and the uniform distribution. As a way to make the mutual-information loss more tolerant to imbalanced distributions the authors of \cite{alphaTIM} proposed a relaxed version based on $\alpha-$divergences. Leveraging Tsallis $\alpha$-divergence \cite{alphaTIM} proposes an $\alpha$-mutual information term defined as:
\begin{equation}
\begin{split}
    \mathcal{I}_{\alpha}(X_Q; Y_Q) & \defn \mathcal{H}_{\alpha} - \mathcal{H}_{\alpha}(Y_Q|X_Q)\\
    & = \frac{1}{\alpha-1}\left(\frac{1}{M}\sum_{i\in Q}\sum_{j=1}^N (p^{q}_{ij})^{\alpha} -\sum_{j=1}^N(\hat{p}^{q}_j)^{\alpha}\right)\\
    \end{split}
    \label{eq:alpha_MI}
\end{equation}

The reader is advised to see section 5 from \cite{alphaTIM} regarding the derivation and analysis of the above term. In a similar way to the balanced loss term \eq{balanced}, in the imbalanced setting we minimize the final loss function with respect to $\Phi$ defined as:
\begin{equation}
    L_{imbal}(S;Q) \defn L_{ce}(X_S; Y_S) -\mathcal{I}_{\alpha}(X_Q; Y_Q)%+  \lambda_2\mathcal{H}(Y_Q|X_Q) -\lambda_3\mathcal{H}(Y_Q)%-\lambda_1\frac{1}{|S|}\sum_{i\in S}\sum_{k=1}^Ky_{ik}\log(p_{ik}) -\big\displaystyle(-\sum_
\label{eq:imbalanced}
\end{equation}
\subsection{Iterative Manifold parameters optimization}
\label{sec:manifold_adaptation}
In contrast to \cite{TIM} and \cite{alphaTIM}, rather than only optimizing the class centroids, we optimize the whole set of manifold parameters $\Phi$ which includes the class centroids, $\mathcal{C}$ as well as graph specific parameters such as $\mathcal{B}$ and $\mathcal{G}$. Since we use a differentiable loss function we can update the manifold parameters $\Phi$ by minimizing \eq{balanced} or \eq{imbalanced} through any gradient-based optimization algorithm. The procedure from graph construction, section \ref{sec:graph_contruction}, to manifold parameter optimization, section \ref{sec:manifold_adaptation}, is iterated until convergence.
\subsection{Transductive Inference}
\label{sec:transductive_inference}

Upon convergence of the manifold parameters $\Phi$, we calculate the final manifold similarity matrix $Z$ and use the last M rows to obtain the submatrix $Z^Q$ that provides manifold class similarity values for the set $Q$. Finally, for each query $x_{i}$, $i \in [M]$, we predict the \emph{pseudo-label}

\begin{equation}
	 \hat{y}_{i} \defn \arg\max_{j \in [N]} Z_{ij}
\label{eq:argmax}
\end{equation}
that corresponds to the maximum element of the $i$-th row of $Z^Q$, for $i \in [M]$.




==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/related-1.tex <==
\section{Related work}
\label{sec:related}

\subsection{Few-shot learning}
Learning from limited data as a problem has troubled the computer vision and machine learning community for a long time \cite{one_shot_start}. A large proportion of the current approaches addressing few-shot learning focus on the meta-learning paradigm. Meta-learning methods can be roughly partitioned into three distinct approaches, model-based \cite{SNAIL, santoro, metaNet, hypernetworks},  optimization based meta-learning \cite{MAML, reptile, iMAML, LEO}  and metric-based \cite{matchingNets, prototypical, siamese, relationnet} . Model-based meta-learning methods utilize specialized networks such as memory augmented neural networks \cite{santoro} and meta-networks \cite{metaNet} to aid the meta-learning process. Optimization-based methods focus on learning a robust model initialization, this can be learned through gradient-based solutions \cite{MAML, reptile}, closed-form solutions\cite{bertinetto} or even through an LSTM \cite{ravilstm}. Metric-based approaches work on the embedding space by calculating the similarities of a query example with class centroids \cite{prototypical}, utilizing a learnt similarity function \cite{relationnet} or using siamese networks to compare pairs of images \cite{siamese}.%Initially, learning from limited data was explored through the paradigm of meta-learning \cite{schmidhuber_l2l, thrun_l2l}. Cu


Recent works such as \cite{rfs, closerlook} have shown that the transfer learning paradigm can outperform meta-learning methods. Transfer learning methods decouple the training phase from the inference stage and aim at learning powerful representations through the use of well designed pre-training regimes to train the backbone network. The pre-training regime can train a model with auxiliary loss functions along with the standard cross entropy loss such as such as knowledge-distillation \cite{rfs}, Manifold Mixup \cite{manifoldmixup} and other self-supervised learning loss functions such as predicting rotations \cite{gidarisRot} and instance contrastive learning \cite{fsl_contrastive}.

Another way to address the data deficiency of few-shot learning is to augment the support set with synthetic data. Synthetic data can be generated either in the image space or in the feature space through the use of a \emph{hallucinator} trained on the base classes. The hallucinator could be trained following common generative models such as \emph{Generative Adversarial Networks} (GANs) \cite{metaGAN, AFHN, funit}
and \emph{Variational Autoencoders} (VAEs) \cite{VIFSL}. Other works proposed hallucinators specifically designed for the few-shot learning paradigm \cite{Ideme, salnet, DTN, TFH}.
 


\subsection{Transductive few-shot learning}
Transductive few-shot learning studies few-shot learning in the case where all queries are available and can be utilized to improve the classification performance at inference time. Many methods exploit the data manifold through the use of label propagation \cite{ilpc, local_lp}, embedding propagation \cite{embeddingpropagation} or by taking advantages of Riemannian geometry through the use of the oblique manifold \cite{oblique_manifold}. Another direction explores ways of using both labeled and unlabelled examples to improve the class centroids. For example, \cite{pt_map} use soft k-means to iteratively update the class centroids, \cite{BDCSPN} carry out prototype rectification by minimizing the cross-class and intra-class variance while \cite{TIM} iteratively adapts the class centroids by maximizing the mutual information between query features and their label predictions. Other methods explored ways of iteratively selecting the most confident pseudo-labeled queries, for example by interpreting the pseudo-label selection as label denoising \cite{ilpc} or by calculating the credibility of each pseudo-label \cite{lrici}. %Other noteworthy methods include learning a discriminative subspace through dimensionality reduction \cite{tafssl} and meta-learning a scaling function \cite{mct}.

\subsection{Perfectly class-balanced tasks}
\label{sec:cls_bal}
As it was stated in section \ref{sec:intro} it has been argued in \cite{alphaTIM} that the commonly used transductive few-shot learning benchmarks use perfectly class-balanced tasks and several methods exploit this bias by utilizing class balancing techniques improving their performance in the process. \cite{pt_map} and \cite{ilpc} achieved remarkable performances by optimizing the query probability matrix, $P$ to have specific row and column sums of $\vp$ and $\vq$ respectively. The row sum $\vp$ amounts to the probability distribution of every query while the column sum corresponds to the total number of examples per class. By iteratively normalizing every row and column to sum to $\vp$ and $\vq$ respectively through the Sinkhorn-Knopp algorithm and setting $\vq$ equal to the number of queries per class the prior knowledge of the distribution of examples per class can be exploited. Specifically \cite{ilpc} gained $\sim 1-2\%$ and $\sim 5\%$ in 1-shot and 5-shot setting respectively through this technique.

Class-balancing is also used in \cite{TIM} through the use of the mutual-information maximization loss function. The proposed loss function is composed of three terms, the cross-entropy loss, the conditional entropy loss and the label-marginal entropy loss. The label-marginal entropy loss encourages the distribution of predicted labels to follow a uniform distribution, in other words it encourages the model to converge to class-balanced solutions.








